Projection: A Unified Approach to Semi-Infinite Linear Programs and Duality in Convex Programming

Fourier-Motzkin elimination is a projection algorithm for solving finite linear programs. We extend Fourier-Motzkin elimination to semi-infinite linear programs which are linear programs with finitely many variables and infinitely many constraints. Applying projection leads to new characterizations of important properties for primal-dual pairs of semi-infinite programs such as zero duality gap, feasibility, boundedness, and solvability. Extending the Fourier-Motzkin elimination procedure to semi-infinite linear programs yields a new classification of variables that is used to determine the existence of duality gaps. In particular, the existence of what the authors term dirty variables can lead to duality gaps. Our approach has interesting applications in finite-dimensional convex optimization. For example, sufficient conditions for a zero duality gap, such as existence of a Slater point, are reduced to guaranteeing that there are no dirty variables. This leads to completely new proofs of such sufficient conditions for zero duality.

==> application-conic.tex <==
% !TEX root = ../fm-paper-resubmit-again.tex
\section{Application: Conic linear programs}\label{s:application-conic}

In conic programming the standard primal is
%
\begin{align*}\label{eq:conlp-primal}
\begin{array}{rl}
\quad \inf_{x\in X} & \langle x, \phi  \rangle \\
\textrm{s.t.} & A(x) \succeq_P d
\end{array}\tag{\text{ConLP}}
\end{align*}
%
where $X$ is a finite dimensional vector space and $Y$ an arbitrary vector space, $A : X \rightarrow Y$ is a linear mapping, $d \in Y$, $P$ is a pointed convex cone in $Y$ and $\phi$ is a linear functional on $X$. The standard dual (also a conic program) is
%
\begin{align*}\label{eq:conlp-dual}
\begin{array}{rl}
\sup_{\psi \in Y'} & \langle d, \psi  \rangle \\
\textrm{s.t.} & A'(\psi) = \phi \\
& \psi \in P'.
\end{array}\tag{\text{ConLPD}}
\end{align*}
%
We study a semi-infinite linear program that is equivalent to (ConLP) and use the method of projection to give a new proof of the following well-known duality result for conic programs. 
%
\theoremstyle{definition}
\newtheorem*{thm:slater}{Theorem~\ref{thm:slater}}
\begin{thm:slater}[Zero duality gap via an interior point]
Let $X$ and $Y$ be finite-dimensional vector spaces, and let $P$ be reflexive. Assume the primal conic program~\eqref{eq:conlp-primal} is feasible. Suppose there exists a $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi$. Then the primal-dual pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual} has a zero duality gap. Moreover, the primal is solvable.
\end{thm:slater}
%
Our proof uses the interior point $\psi^*$ to construct a set of  constraints that show the associated semi-infinite linear program is tidy. Thus,  zero duality gap and primal solvability are established in a transparent ``algebraic" manner. 
We believe our results add fresh insight to the literature on connections between conic programming and semi-infinite linear programming (see, for instance Zhang \cite{zhang2010understanding}).

Recall the definition of \eqref{eq:conlp-primal} in Section~\ref{s:introduction} and its standard dual \eqref{eq:conlp-dual}. 
%They are reproduced here for convenience. The conic  primal is
%\begin{align*}
%\begin{array}{rl}
%\quad \inf_{x\in X} & \langle x, \phi  \rangle \\
%\textrm{s.t.} & A(x) \succeq_P d
%\end{array}\tag{\text{ConLP}}
%\end{align*}
%where $X$ and $Y$ are vector spaces, $A : X \rightarrow Y$ is a linear mapping, $d \in Y$, $P$ is a pointed convex cone in $Y$ and $\phi$ is a linear functional on $X$. The conic dual is
%\begin{align*}
%\begin{array}{rl}
%\sup_{\psi \in Y'} & \langle d, \psi  \rangle \\
%\textrm{s.t.} & A'(\psi) = \phi \\
%& \psi \in P'.
%\end{array}\tag{\text{ConLPD}}
%\end{align*}
%We apply our methodology to an important class of problems: conic linear programs, 
%\begin{align*}\label{eq:conlp-primal}
%\begin{array}{rl}
%\quad \inf_{x\in X} & \langle x, \phi  \rangle \\
%\textrm{s.t.} & A(x) \succeq_P d
%\end{array}\tag{\text{ConLP}}
%\end{align*}
%with two linear vector spaces $X, Y$, a linear mapping $A : X \rightarrow Y$, a vector $d \in Y$, a pointed convex cone
%%\footnote{\texttt{TODO: define precisely what we mean by pointed}}  
%$P \subseteq Y$ and a linear functional $\phi \in X'$.   Denote the dual cone of $P$ by $P' = \{\psi \in Y' \st \langle y, \psi\rangle \geq 0 \textrm{ for all } y \in P\}$.  Define the algebraic adjoint $A' : Y' \rightarrow X'$,  by $\langle A(x), \psi \rangle = \langle x, A'(\psi) \rangle$ for every $x \in X$ and $\psi \in Y'$. The dual problem to \equerry{eq:conlp-primal} is:
%
%\begin{align*}\label{eq:conlp-dual}%
%\begin{array}{rl}
%\sup_{\psi \in Y'} & \langle d, \psi  \rangle \\
%\textrm{s.t.} & A'(\psi) = \phi \\
%& \psi \in P'
%\end{array}\tag{\text{ConLPD}}
%\end{align*}
%
Let $F = \{x \in X\st A(x) \succeq_P d\}$ denote the feasible region of \eqref{eq:conlp-primal}. In our development, it is convenient to assume that the algebraic adjoint $A'$ of linear map $A$ is surjective (in order to apply the Open Mapping Theorem, see below). We show in the Electronic Companion (Lemmas~\ref{lem:A'-surjective}--\ref{lem:restriction-problem} and Remark~\ref{rem:surjective-assum}) this can be assumed without out loss of generality when \eqref{eq:conlp-primal} is feasible and bounded. 

%For any linear map $T$ defined on $X$, let $\ker(T) = \{x \in X : T(x) = 0\}$ denote the kernel of $T$.
%
%% find this result in functional analysis text. Note that this result does not hold for topological adjoints necessarily. This is discussed in Luenberger. See also 
%%http://math.stackexchange.com/questions/269105/t-surjective-iff-t-injective-in-infinite-dimensional-hilbert-space
%\begin{lemma}\label{lem:A'-surjective}
%Given a linear mapping  $A:X \rightarrow Y$,  $\ker(A) = \{0\}$ if and only if $A'$ is surjective.
%\end{lemma}
%\begin{proof}
%($\Longrightarrow$)  If  $\ker(A) = \{0\}$, then $A$ is one-to-one and there is  a linear map $A^{-1} : Im(A) \to X$.  Let $\phi$ be an arbitrary linear functional in  $X^{\prime}.$  We show there exists a linear functional $\psi \in Y^{\prime}$  such that   $\phi = A^{\prime}(\psi).$    Define the linear functional $\phi \circ A^{-1}$  on $Im(A)$ and let  $\psi$ be any extension of this linear functional  from  $Im(A)$ to $Y$. Thus $\psi \in Y'$. We now show $\phi = A'(\psi)$. For any $x \in X$, $\langle x, A'(\psi)\rangle = \langle A(x), \psi \rangle = (\phi \circ A^{-1} )(A(x)) = \phi(x) = \langle x, \phi \rangle$. The second equality follows since $A(x) \in Im(A)$.
%
%($\Longleftarrow$) Consider $x \in X$ such that $A(x) = 0$. Note that for every $\phi \in X'$, $\langle x, \phi \rangle = 0$. This would imply that $x = 0$. Since $A'$ is surjective, for every $\phi \in X'$ there exists $\psi \in Y'$ such that $A'(\psi) = \phi$. Thus, $\langle x, \phi \rangle = \langle x, A'(\psi) \rangle = \langle A(x), \psi \rangle = \langle 0, \psi \rangle = 0$. \end{proof}
%
%\begin{lemma}\label{lem:kernel} If \eqref{eq:conlp-primal} is feasible and bounded, then $\ker(A) \subseteq \ker(\phi)$. 
%\end{lemma}
%\begin{proof}
%Prove the contrapositive and assume  that there is an  $r \in \ker(A) \setminus \ker(\phi)$. Without loss of generality assume $\langle r, \phi \rangle < 0$ (otherwise  make the argument with $-r$). Let $\bar x$ be a feasible solution to \eqref{eq:conlp-primal}, i.e., $A(\bar x) \succeq_P d$. Since $r \in \ker(A)$,  $A(\bar x + \lambda r) \succeq_P d$ for all $\lambda \geq 0$. But since $\langle r, \phi \rangle < 0$, $\langle \bar x + \lambda r, \phi \rangle \to -\infty$ as $\lambda \to \infty$, contradicting the boundedness of \eqref{eq:conlp-primal}.\end{proof}
%
%\begin{lemma}\label{lem:restriction-problem}
%Let $X$ be a finite-dimensional space, so that orthogonal complements of subspaces are well-defined. Let $\bar\phi = \phi|_{\ker(A)^\perp}$ be the linear functional  on $\ker(A)^\perp$ defined by the restriction of $\phi$ to $\ker(A)^\perp$. Similarly, let $\bar A = A|_{\ker(A)^\perp}$ denote the restriction of the linear map $A$. Consider the optimization problem 
%
%\begin{equation}\label{eq:conlp-primal-lineality}
%\begin{array}{rl}
%\quad \inf_{x\in \ker(A)^\perp} & \langle x, \bar\phi  \rangle \\
%\textrm{s.t.} & \bar A(x) \succeq_P d.
%\end{array}
%\end{equation}
%%
%If \eqref{eq:conlp-primal} is feasible and bounded, the optimal value of \eqref{eq:conlp-primal} equals the optimal value of~\eqref{eq:conlp-primal-lineality}. Moreover, if $O$ is the set of optimal primal solutions for \eqref{eq:conlp-primal}, and $\overline O$ is the set of optimal primal solutions for~\eqref{eq:conlp-primal-lineality}, then $O = \overline O + \ker(A)$. 
%\end{lemma}
%
%\begin{proof}
%Since \eqref{eq:conlp-primal} is feasible and bounded,  $\ker(A) \subseteq \ker(\phi)$ by Lemma~\ref{lem:kernel}. For any $x$ feasible to \eqref{eq:conlp-primal}, let $r \in \ker(A)$ and $\bar x \in \ker(A)^\perp$ such that $x = \bar x + r$. Since $\ker(A) \subseteq \ker(\phi)$, $\langle r, \phi \rangle = 0$. Thus, $\langle x, \phi\rangle = \langle \bar x + r, \phi \rangle = \langle \bar x, \phi \rangle = \langle \bar x, \bar \phi \rangle$, the last equality follows since $\bar x \in \ker(A)^\perp$. Similarly, $\bar A(\bar x) = A(\bar x) = A(\bar x + r) = A(x) \succeq_P d$. Thus, $\bar x$ is a feasible solution to~\eqref{eq:conlp-primal-lineality} with the same objective value as $\langle x, \phi \rangle$. 
%\end{proof}
%
%\begin{remark}\label{rem:surjective-assum}
%By Lemma~\ref{lem:restriction-problem}, when \eqref{eq:conlp-primal} is feasible and bounded, it suffices to consider a restricted optimization problem like~\eqref{eq:conlp-primal-lineality}. Note that $\ker(\bar A) = \{0\}$. Thus, without loss of generality,  it is valid to assume that for an instance of a feasible and bounded \eqref{eq:conlp-primal} in a finite-dimensional space $X$, the linear map $A$ has zero kernel, i.e., it is one-to-one. This implies that $A'$ is surjective by Lemma~\ref{lem:A'-surjective}. \hfill$\triangleleft$
%\end{remark}

Construct the following primal-dual pair of semi-infinite linear programs in the case where $X$ is finite-dimensional and the cone $P$ is reflexive.  Recall that a cone $P$ is  {\em reflexive} if $P'' = P$ under the natural embedding of $Y \hookrightarrow Y''$. The condition that $P$ is reflexive naturally holds in many important special cases of conic programming.   Once such case is when  $X$ and $Y$ are  finite dimensional spaces and $P$ is a closed, pointed cone in $Y$.   Then $P$ is easily seen to be reflexive. This case includes   linear programming, semi-definite programming (SDPs) and copositive programming. The above reformulation as a semi-infinite linear program works for any such instance.

%The significance of this property will become apparent in Theorem~\ref{theorem:new_express}. 
The primal semi-infinite linear program is
%
\begin{align*}\label{eq:con-silp}
\begin{array}{rl}
\quad \inf_{x \in \R^n}  & c^\top x  \\
\textrm{s.t.} & a^1(\psi)x_1 + a^2(\psi)x_2 + \cdots + a^n(\psi)x_n \geq   b(\psi) \quad \text{ for all } \psi \in P'
\end{array}\tag{\text{ConSILP}} 
\end{align*}
where $X$ is isomorphic to $\R^n$ with respect to a basis $e^1, \ldots, e^n$ and  $c \in \R^n$ represents the linear functional $\phi \in X'$ (also using the isomorphism of $X'$ and $\R^n$).  In \eqref{eq:con-silp}, the elements $a^{j} \in \R^{P^{\prime}}$  $j = 1, \ldots, n$ and $b \in \R^{P^{\prime}},$ are defined by $a^j(\psi) := \langle A(e^j), \psi \rangle$ and $b(\psi) := \langle b, \psi \rangle$. The finite support dual of \eqref{eq:con-silp} is
\begin{align*}\label{eq:con-silp-lagrangian-dual-finite}
\begin{array}{rcl}
\sup \sum_{\psi \in P'} b(\psi) v(\psi) && \\
 \quad  {\rm s.t.} \quad \sum_{\psi \in P'} a^{k}(\psi) v(\psi) &=& c_k\quad \text{ for } k = 1, \ldots, n \\
v &\in& \R^{(P')}_+.
\end{array}\tag{\text{ConFDSILP}}
\end{align*}
%
The close connection of this primal-dual pair to the conic pair  \eqref{eq:conlp-primal}--\eqref{eq:conlp-dual} is shown in Theorem~\ref{theorem:new_express} and Theorem~\ref{theorem:new_express_dual} of the Electronic Companion. Theorem~\ref{theorem:new_express} shows that \eqref{eq:conlp-primal} and 
\eqref{eq:con-silp} are \emph{equivalent}, meaning their respective feasible sets are isomorphic under an isomorphism which preserves objective values. In particular, this means $v(\ref{eq:conlp-primal}) = v(\ref{eq:con-silp})$. Similarly, Theorem~\ref{theorem:new_express_dual} shows that \eqref{eq:conlp-dual} and \eqref{eq:con-silp-lagrangian-dual-finite} are equivalent. In particular this means, $v(\ref{eq:conlp-dual})=v(\ref{eq:con-silp-lagrangian-dual-finite})$.

%\begin{theorem}[Primal correspondence]\label{theorem:new_express} 
%Assume $P$ is reflexive and $X$ is finite-dimensional. Let $e^1, \ldots, e^n$ be the basis of $X$ used to define~\eqref{eq:con-silp} and ~\eqref{eq:con-silp-lagrangian-dual-finite}. Then, $v(\ref{eq:conlp-primal}) = v(\ref{eq:con-silp})$. Moreover, the set of feasible solutions to \eqref{eq:conlp-primal} is isomorphic to the set of feasible solutions to \eqref{eq:con-silp} under this basis.
%\end{theorem}
%\begin{proof}
%Since $X$ is isomorphic to $\R^n$ with respect to the basis $e^1, \ldots, e^n$  and  $c \in \R^n$  represents the linear functional $\phi \in X'$ the objective functions of both problems are identical (under this isomorphism). The result  follows if the feasible regions of both problems are isomorphic under this same mapping. 
%%
%%We view $X$ as isomorphic to $\R^n$ under a fixed basis $e^1, \ldots, e^n$. If $P$ is reflexive, then the feasible region $F$ of~\eqref{eq:conlp-primal}  is expressed, using (possibly infinitely many) linear inequalities in $\R^n$, as  $$F = \{x\in \R^n\st \sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle \quad \forall \psi \in P'\},$$
%
%Let $F$ denote the feasible region of (ConLP) and $\hat F$ denote the feasible region of (ConSILP). We show $F$ is isomorphic to $\hat F$ under the basis $e^1, \ldots, e^n$. 
%%
%%Let $\hat F = \{x\in \R^n\st \sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle \quad \forall \psi \in P'\}$.   
%First we show that if $x = x_1e^1 + \ldots + x_ne^n \in F$ then $(x_1, \ldots, x_n) \in \hat F$.   If $x\in F$, then  $A(x) \succeq_P d$. Therefore, $A(x) - d \in P$ and so for all $\psi \in P'$, $ \langle (A(x) - d), \psi \rangle \geq 0$. Writing $A(x) = \sum_{j=1}^n x_j A(e^j)$ and using the linearity of $\psi$, it follows  that $(x_1, \ldots, x_n)\in \hat F$.
%
%Next we show that if $(x_1, \ldots, x_n) \in \hat F$, then $x = x_1e^1 + \ldots + x^ne^n \in F$.  We establish the contrapositive, i.e. if $x \not\in F$ then $(x_1, \ldots, x_n) \not\in \hat F$. If $x \not\in F$,  then $A(x) - d \not\in P$ and since $P$ is reflexive, $A(x)-d \not\in P''$ (under the natural embedding of $Y \hookrightarrow Y''$). Therefore, there exists $\psi  \in P'$ such that $\langle (A(x)-d), \psi \rangle < 0$. Again, using the linearity of $\psi$  it follows  that $(x_1, \ldots, x_n) \not\in \hat F$.
%\end{proof}

%Let $X$ be a finite-dimensional vector space. We view $X$ as isomorphic to $\R^n$ under a fixed basis $e^1, \ldots, e^n$. If $P$ is reflexive, then the feasible region $F$ of~\eqref{eq:conlp-primal}  is expressed, using (possibly infinitely many) linear inequalities in $\R^n$, as  $$F = \{x\in \R^n\st \sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle \quad \forall \psi \in P'\},$$
%\end{theorem}

%One can convert an instance of \eqref{eq:conlp-primal} into an instance of \eqref{eq:SILP} under certain assumptions. Recall that a cone $P$ is  {\em reflexive} if $P'' = P$ under the natural embedding of $Y \hookrightarrow Y''$. %Note that since $P'' = P$ the dual of (6.2) is (6.1). 

%\begin{theorem}\label{theorem:new_express} [Primal Correspondence]
%Let $X$ be a finite-dimensional vector space. We view $X$ as isomorphic to $\R^n$ under a fixed basis $e^1, \ldots, e^n$. If $P$ is reflexive, then the feasible region $F$ of~\eqref{eq:conlp-primal}  is expressed, using (possibly infinitely many) linear inequalities in $\R^n$, as  $$F = \{x\in \R^n\st \sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle \quad \forall \psi \in P'\},$$
%\end{theorem}
%\begin{proof}
%Let $\hat F = \{x\in \R^n\st \sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle \quad \forall \psi \in P'\}$.   First show $F \subseteq \hat F$.   If $x\in F$, then  $A(x) \succeq_P d$. Therefore, $A(x) - d \in P$ and so for all $\psi \in P'$, $ \langle (A(x) - d), \psi \rangle \geq 0$. Writing $A(x) = \sum_{j=1}^n x_j A(e^j)$ and using the linearity of $\psi$, it follows  that $x\in \hat F$.
%
%Next  show that $\hat F \subseteq F$.  Show the contrapositive, i.e. if $x \not\in F$ then $x \not\in \hat F$. If $x \not\in F$,  then $A(x) - d \not\in P$ and since $P$ is reflexive, $A(x)-d \not\in P''$ (under the natural embedding of $Y \hookrightarrow Y''$). Therefore, there exists $\psi  \in P'$ such that $\langle (A(x)-d), \psi \rangle < 0$. Again, using the linearity of $\psi$  it follows  that $x \not\in \hat F$.
%\end{proof}

%Theorem~\ref{theorem:new_express}  implies  \eqref{eq:conlp-primal} is equivalent to  an instance of \eqref{eq:SILP} when $X$ is finite-dimensional and $P$ is reflexive.  The equivalent problem is
%\begin{align*}\label{eq:con-silp}
%\begin{array}{rl}
%\quad \inf_{x \in \R^n}  & c^\top x  \\
%\textrm{s.t.} & a^1(\psi)x_1 + a^2(\psi)x_2 + \ldots + a^n(\psi)x_n \geq   b(\psi) \quad \forall \psi \in P'
%\end{array}\tag{\text{ConSILP}} 
%\end{align*}
%where $X$  is isomorphic to $\R^n$ (with respect to a basis $e^1, \ldots, e^n$), and use the shorthand notation $c \in \R^n$ to denote the linear functional $\phi \in X'$ (also using the isomorphism of $X'$ and $\R^n$).  In \eqref{eq:con-silp}, the elements $a^{j} \in \R^{P^{\prime}}$  $j = 1, \ldots, n$ and $b \in \R^{P^{\prime}},$ are defined by $a^j(\psi) := \langle A(e^j), \psi \rangle$ and $b(\psi) := \langle d, \psi \rangle$.

%\begin{example}
%Consider the following semidefinite program
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \quad  x
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right]
%+
%t
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right]
%&\succeq& 
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right]
%\end{eqnarray*}
%
%
%The dual problem is
%\begin{eqnarray*}
%\sup 
%\left<
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right] ,
%\psi   \right> \\
%{\rm s.t.} \qquad 
%\left<
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right] ,
%\psi   \right>  = 0\\
%\left<
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right] ,
%\psi   \right>  = 1 \\
%\psi \succeq 0
%\end{eqnarray*}
%Now formulate \eqref{eq:con-silp}.
%
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \qquad x 
%\left<
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right] ,
%\psi   \right> 
%+
%t
%\left<
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right] ,
%\psi   \right>
%&\ge&
%\left<
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right] ,
%\psi   \right> 
%\end{eqnarray*}
%This simplifies to
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \qquad  
%x \psi_{11} + t \psi_{22} 
%&\ge& -2 \psi_{12}
%\end{eqnarray*}
%This simplifies to
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad   z - t &\ge& 0 \\
%x \psi_{11} + t \psi_{22} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} > 0 \\
%x \psi_{11} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%t \psi_{22} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} = 0, \psi_{22} > 0 
%\end{eqnarray*}
%Project out the $t$ variable. This gives
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0  \\
%x \psi_{11} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%z  
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} =  0, \psi_{22} > 0 
%\end{eqnarray*}
%Now for the $\psi$ to be positive semidefinite, if either $\psi_{11} = 0$ or $\psi_{22} = 0$, the $\psi_{12} = 0$ so the system becomes
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0  \\
%x \psi_{11} 
%&\ge& 0, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%z  
%&\ge&  0,  \quad \psi_{11} =  0, \psi_{22} > 0 
%\end{eqnarray*}
%Dividing the second inequality by the strictly positive $\psi_{11}$ gives
%\begin{eqnarray}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0   \label{eq:cone-I4}\\
%x 
%&\ge& 0, \quad \psi_{11} > 0, \psi_{22} = 0  \label{eq:cone-I2}\\
%z  
%&\ge&  0,  \quad \psi_{11} =  0, \psi_{22} > 0 \label{eq:cone-I3}
%\end{eqnarray}
%In this system, equations (\ref{eq:cone-I4}) correspond to the set $I_{4}$ in (\ref{eq:J_system}),  equations (\ref{eq:cone-I2}) correspond to the set $I_{2}$ in (\ref{eq:J_system}), and equations (\ref{eq:cone-I3}) correspond to the set $I_{3}$ in (\ref{eq:J_system}).
%So now 
%\begin{eqnarray*}
%\omega(\delta) = \sup \{ - \frac{2 (\psi_{12} + \delta \psi_{11})}{\psi_{22}}  \, : \,  \psi_{11}, \psi_{22} \ge 0\}
%\end{eqnarray*}
%Now look at slide IMG\_0083.jpg.  We argue you can take $\psi_{11} = 1.$  Since the matrix $\psi$ must be positive semidefinite, $\psi_{11} \psi_{22} - \psi_{12} \psi_{21} \ge 0.$  Then taking  $\psi_{11} = 1$ gives  $\psi_{22} - \psi_{12} \psi_{21} \ge 0.$ But the $\psi$ matrix is positive symmetric so $\psi_{22} \ge \psi_{12}^{2}.$  Then
%\begin{eqnarray*}
%\frac{-2 \psi_{12} - \delta}{\psi_{22}} \le  \frac{-2 \psi_{12} - \delta}{\psi_{12}^{2}}
%\end{eqnarray*}
%Optimizing by Calculus  gives $\psi_{12} = \delta$ and we get $(\delta) \le \frac{1}{\delta}.$ \hfill$\triangleleft$
%\end{example}



%Now show that the finite support dual of \eqref{eq:con-silp} corresponds in a well-defined manner to the conic dual program~\eqref{eq:conlp-dual}.  The finite support dual of~\eqref{eq:con-silp} is 
%\begin{align*}\label{eq:con-silp-lagrangian-dual-finite}
%\begin{array}{rcl}
%\sup \sum_{\psi \in P'} b(\psi) v(\psi) && \\
% \quad  {\rm s.t.} \quad \sum_{\psi \in P'} a^{k}(\psi) v(\psi) &=& c_k, \quad k = 1, \ldots, n \\
%v &\ge& 0, \quad v \in \R^{(P')}
%\end{array}\tag{\text{ConFDSILP}}
%\end{align*}

%\begin{theorem}[Dual Correspondence]\label{theorem:new_express_dual}
% Assume $P$ is reflexive and $X$ is finite-dimensional. Let $e^1, \ldots, e^n$ be the basis of $X$ used to define~\eqref{eq:con-silp} and ~\eqref{eq:con-silp-lagrangian-dual-finite}. Then, $v(\ref{eq:conlp-dual}) = v(\ref{eq:con-silp-lagrangian-dual-finite})$. Moreover, there exists maps $T : P' \to \R^{(P')}_+$ and $\hat T : \R^{(P')}_+ \to P'$ such that if $\psi \in P'$ is a feasible solution to \eqref{eq:conlp-dual} then $T(\psi)$ is a feasible solution to \eqref{eq:con-silp-lagrangian-dual-finite}.  Conversely, if $v \in \R^{(P')}$ is a feasible solution to \eqref{eq:con-silp-lagrangian-dual-finite} then $\hat T(v)$ is a feasible solution to \eqref{eq:conlp-dual}.
%\end{theorem}
%\begin{proof}
%It suffices to construct maps $T$ and $\hat T$ which satisfy the following properties.
%\begin{enumerate}[(i)]
%\item $\langle e^k, A'(\psi^*)\rangle = \sum_{\psi \in P'} a^{k}(\psi) T(\psi^*)(\psi)$, for every $\psi^* \in P'$ and all $k=1, \ldots, n$.
%\item $\langle d, \psi^* \rangle = \sum_{\psi \in P'}b(\psi)T(\psi^*)(\psi)$, for every $\psi^* \in P'$.
%\item $\sum_{\psi \in P'} a^{k}(\psi) v(\psi) = \langle e^k, A'(\hat T(v))\rangle$, for every $v \in \R^{(P')}_+$ and all $k=1, \ldots, n$.
%\item $\sum_{\psi \in P'}b(\psi)v(\psi) = \langle d, \hat T(v) \rangle$, for every $v \in \R^{(P')}_+$.
%\end{enumerate}
%%
%The map $T$ is defined as follows. For any $\psi^* \in P'$, $T(\psi^*)$ is the finite support element $v^* \in \R^{(P')}$ where the only non-zero component of $v^*$ is 1 and corresponds to $\psi^*$. For any $k \in \{1, \ldots, n\}$, $\sum_{\psi \in P'} a^{k}(\psi) v^*(\psi) = a^k(\psi^*) = \langle A(e^k), \psi^* \rangle = \langle e^k, A'(\psi^*) \rangle$ and  (i) is satisfied.  Also,  $\sum_{\psi \in P'}b(\psi)v^*(\psi) = b(\psi^*)=\langle d, \psi^* \rangle$ and  (ii) is satisfied.
%
%The map $\hat T$ is defined as follows. For any $v^* \in \R^{(P')}$, $\hat T(v^*) = \sum_{\psi\in P'}v^*(\psi)\psi$ where the sum is well-defined because $v^*$ has finite support. Since $v^*$ has nonnegative entries, $\hat T(v^*) \in P'$. Now, $\sum_{\psi \in P'} a^k(\psi)v^*(\psi) = \sum_{\psi \in P'}\langle A(e^k), \psi \rangle v^*(\psi) = \langle A(e^k), \sum_{\psi \in P'} v^*(\psi)\psi\rangle = \langle A(e^k), \hat T(v^*) \rangle = \langle e^k, A'(\hat T(v^*)\rangle$ and (iii) is satisfied.  Also, $\sum_{\psi \in P'}b(\psi)v^*(\psi) = \sum_{\psi \in P'} \langle d, \psi\rangle v^*(\psi) = \langle d, \sum_{\psi \in P'}v^*(\psi)\psi \rangle = \langle d, \hat T(v^*)\rangle$ and (iv) is satisfied.
%\end{proof}
%
%\begin{theorem}[Dual Correspondence]\label{theorem:new_express_dual}
%Suppose $P$ is reflexive and $X$ is finite-dimensional and let $e^1, \ldots, e^n$ be a basis of $X$ under which we form~\eqref{eq:con-silp} and ~\eqref{eq:con-silp-lagrangian-dual-finite}. Let $\R^{(P')}_+$ denote the set $\{v \in \R^{(P')} : v \geq 0\}$. There exist maps $T : P' \to \R^{(P')}_+$ and $\hat T : \R^{(P')}_+ \to P'$ satisfying the following properties.
%\begin{enumerate}
%\item $\langle e^k, A'(\psi^*)\rangle = \sum_{\psi \in P'} a^{k}(\psi) T(\psi^*)(\psi)$, for every $\psi^* \in P'$ and all $k=1, \ldots, n$.
%\item $\langle d, \psi^* \rangle = \sum_{\psi \in P'}b(\psi)T(\psi^*)(\psi)$, for every $\psi^* \in P'$.
%\item $\sum_{\psi \in P'} a^{k}(\psi) v(\psi) = \langle e^k, A'(\hat T(v))\rangle$, for every $v \in \R^{(P')}_+$ and all $k=1, \ldots, n$.
%\item $\sum_{\psi \in P'}b(\psi)v(\psi) = \langle d, \hat T(v) \rangle$, for every $v \in \R^{(P')}_+$.
%\end{enumerate}
%\end{theorem}
%
%\begin{proof}
%The map $T$ is defined as follows. For any $\psi^* \in P'$, $T(\psi^*)$ is the finite support element $v^* \in \R^{(P')}$ where the only non-zero component of $v^*$ is 1 and corresponds to $\psi^*$. For any $k \in \{1, \ldots, n\}$, $\sum_{\psi \in P'} a^{k}(\psi) v^*(\psi) = a^k(\psi^*) = \langle A(e^k), \psi^* \rangle = \langle e^k, A'(\psi^*) \rangle$; thus 1. is satisfied. Finally, observe that $\sum_{\psi \in P'}b(\psi)v^*(\psi) = b(\psi^*)=\langle d, \psi^* \rangle$; thus, 2. is satisfied.
%
%The map $\hat T$ is defined as follows. For any $v^* \in \R^{(P')}$, $\hat T(v^*) = \sum_{\psi\in P'}v^*(\psi)\psi$ where the sum is well-defined because $v^*$ has finite support. Since $v^*$ has nonnegative entries, $\hat T(v^*) \in P'$. Now, $\sum_{\psi \in P'} a^k(\psi)v^*(\psi) = \sum_{\psi \in P'}\langle A(e^k), \psi \rangle v^*(\psi) = \langle A(e^k), \sum_{\psi \in P'} v^*(\psi)\psi\rangle = \langle A(e^k), \hat T(v^*) \rangle = \langle e^k, A'(\hat T(v^*)\rangle$; thus, 3. is satisfied. Finally observe that $\sum_{\psi \in P'}b(\psi)v^*(\psi) = \sum_{\psi \in P'} \langle d, \psi\rangle v^*(\psi) = \langle d, \sum_{\psi \in P'}v^*(\psi)\psi \rangle = \langle d, \hat T(v^*)\rangle$; thus, 4. is satisfied.\end{proof}

\subsection{Zero duality gap via boundedness}

%We prove Theorem~\ref{thm:tbounded} in this section. 
%A  more  restricted version of the following result is known in the classical conic programming literature (see for example Duffin \cite{duffin1978clark}).   
This result is known in the literature (see for instance Shapiro~\cite{shapiro2005duality}), but we show it as an immediate consequence of Theorem~\ref{theorem:bounded-zero-duality-gap} based on Fourier-Motzkin elimination techniques.

\begin{theorem}[Zero duality gap via boundedness]\label{thm:tbounded}
%Let $X$ be finite-dimensional.  
If $P$ is reflexive and there exists a scalar $\gamma$ such the set $\left\{x : A(x) \succeq_P d \text{ and } \langle x, \phi  \rangle \le \gamma\right\}$ is nonempty and bounded, then there is no duality gap for the primal-dual pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual}.
\end{theorem}

%\begin{proof}
% By Theorem~\ref{theorem:new_express},  the primal optimal value of  \eqref{eq:conlp-primal} is equal to  the optimal value of the \eqref{eq:con-silp}. By Theorem~\ref{theorem:bounded-zero-duality-gap}  there is  a zero duality gap between the primal dual pair~\eqref{eq:con-silp}-\eqref{eq:con-silp-lagrangian-dual-finite}. Finally, from Theorem~\ref{theorem:new_express_dual},  the optimal value of~\eqref{eq:con-silp-lagrangian-dual-finite} is equal to  the optimal value of~\eqref{eq:conlp-dual}.
%\end{proof}

\begin{remark}
The above result shows that semi-definite programs (SDPs) and copositive programs with nonempty, bounded feasible regions have zero duality gap.
\end{remark}

\subsection{Regular duality for conic programs}

We now prove a central result of conic programming, known as {\em regular duality}, using the machinery of FM elimination. First, some notions from conic programming (see Chapter 4 of Gartner and Matous\'ek~\cite{gartner-matousek} for more details). A sequence $(\psi^m)_{m\in \N}$, is called a feasible sequence for the dual program~\eqref{eq:conlp-dual} if $\psi^m \in P'$ for all $m \in \N$ and $\lim_{m \to \infty} A'(\psi^m) = \phi.$

The {\em value of a feasible sequence} $(\psi^m)_{m\in \N}$ is  $\langle d, (\psi^m)_{m\in \N} \rangle = \lim\sup_{m \to \infty}\langle d, \psi^m\rangle$. The {\em limit value (a.k.a. subvalue)} of the dual program~\eqref{eq:conlp-dual} is    $$\sup\{\langle d, (\psi^m)_{m \in \N}\rangle \st (\psi^m)_{m \in \N} \textrm{ is a feasible sequence for }\eqref{eq:conlp-dual} \}.$$
%
%\old{Clearly, the limit value of the dual program is greater than or equal to the optimal value of the dual program, since given a feasible solution $\psi^*$ of the dual, one can consider the feasible sequence where every element of the sequence is $\psi^*$.
%
%\begin{prop}\label{prop:weak-duality-conic}[Weak Duality for Conic Programs (see Theorem 4.7.2 in~Gartner and Matousek~\cite{gartner-matousek})]
%Let $x$ be any feasible solution to the primal conic program~\eqref{eq:conlp-primal} and let $(\psi^k)_{k \in \N}$ be a feasible sequence for the dual program~\eqref{eq:conlp-dual}. Then $\langle x, \phi \rangle \geq \langle d, (\psi^k)_{k \in \N}\rangle$.
%\end{prop} 
%\begin{proof} The proof appears in Gartner and Matousek~\cite{gartner-matousek}; we present it here for completeness.
%$$\begin{array}{rcl}\langle x, \phi \rangle & = & \langle x, \lim_{k\to \infty} A'(\psi^k)\rangle \\
%& = &\lim_{k\to \infty} \langle x,  A'(\psi^k)\rangle \\
%& = & \lim\sup_{k\to \infty} \langle x, A'(\psi^k) \rangle \\
%& = & \lim\sup_{k \to \infty} \langle A(x), \psi^k\rangle \\
%& \geq & \lim\sup_{k \to \infty} \langle d, \psi^k\rangle \\
%& = & \langle d, (\psi^k)_{k\in \N}\rangle
%\end{array}
%$$ where the inequality follows from the fact that $Ax - d \in P$ and $\psi^k \in P'$ for every $k \in\N$.
%\end{proof}
%}
A simple  proof of regular duality for conic programs is easily obtained using projection (see Theorem 4.7.3 in~Gartner and Matousek~\cite{gartner-matousek} for the more standard proof technique).
\begin{theorem}[Regular duality for conic programs]\label{thm:regular-duality}
%Assume $X$ is finite-dimensional and $P$ is reflexive. 
If the primal conic program~\eqref{eq:conlp-primal} is feasible and has a finite optimal value $z^*$,  then the dual program~\eqref{eq:conlp-dual} has a finite limit value $\hat d$ and $z^* = \hat d$.
\end{theorem}
%\old{
%\begin{proof}
%Performing  FM elimination on the \eqref{eq:SILP}~\eqref{eq:con-silp} gives  a system of the form~\eqref{eq:J_system}. By Proposition~\ref{prop:weak-duality-conic},  $\hat d \leq z^*$. Recall the two values that were defined in Section~\ref{s:silp-classification}: $d_1 = \sup\{\tilde b(h): h \in I_3\}$ and $d_2 = \lim_{\delta\to \infty} \omega(\delta)$ where $\omega(\delta)$ is defined in~\eqref{eq:f_delta}. By Lemma~\ref{lemma:primal-optimal-value}, $z^* = \max\{d_1, d_2\}$. 
%
%{\em Case 1: $z^* = d_1$.} By Theorem~\ref{theorem:zero-duality-gap}, $z^* = d^*$ where $d^*$ is the optimal dual value. Since $d^* \leq \hat d \leq z^*$, we have that $\hat d = z^*$.
%
%{\em Case 2: $z^* = d_2$.} By Lemma~\ref{lemma:convergence_lim_case}, there is a sequence $i_m \in I_4$ such that $\lim_{m\to\infty} \tilde b(i_m) = z^*$ and $\lim_{m\to \infty} \tilde a^k(i_m) = 0$ for all $k = 1, \ldots, n$. This sequence corresponds to a feasible sequence for the dual program with value $z^*$. Thus, $\hat d \geq z^*$ and we are done.\end{proof}
%}

\begin{proof}
By Theorem~\ref{theorem:new_express}, the optimal value of~\eqref{eq:con-silp} is equal to  $z^*$ and $z^*$ is finite since the optimal value of~\eqref{eq:conlp-primal} is finite.   By Theorem~\ref{theorem:regular-duality-silp}, the limit value of~\eqref{eq:con-silp-lagrangian-dual-finite} equals the optimal value of~\eqref{eq:con-silp}.   By Theorem~\ref{theorem:new_express_dual},  every feasible sequence 
%$(\psi^m)_{m\in \N}$ 
for~\eqref{eq:conlp-dual} maps  to a feasible sequence 
%$(T(\psi^m))_{m\in \N}$ 
for~\eqref{eq:con-silp-lagrangian-dual-finite}. Similarly, every feasible sequence %$(u^m)_{m\in \N}$ 
for~\eqref{eq:con-silp-lagrangian-dual-finite} 
maps to a feasible sequence 
%$(\hat T(u^m))_{m\in\N}$ 
for~\eqref{eq:conlp-dual}. Thus, the limit value $\hat d$ of~\eqref{eq:conlp-dual} is equal  $z^{*}$,   the limit value of~\eqref{eq:con-silp-lagrangian-dual-finite}.
\end{proof}

%\begin{theorem}\label{thm:slater}[Slater's Condition for Zero Duality Gap]
%Let $X$ and $Y$ be finite-dimensional spaces and assume $P$ is reflexive. If the dual program is strictly feasible, i.e., there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi$. Then we have zero duality gap for the primal-dual pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual}.
%\end{theorem}
%\begin{proof}
%Under the hypothesis, the limit value of the dual is equal to the optimal value of the dual by Theorem 4.6.5 in~\cite{gartner-matousek}. The result then follows from Theorem~\ref{thm:regular-duality}.
%\end{proof}


%\subsection{New Proof of Theorem \ref{thm:slater-mod}}
%
%\begin{theorem}\label{thm:slater-mod}[Slater's Condition for Zero Duality Gap]
%Let $X$ and $Y$ be finite-dimensional spaces and assume $P$ is reflexive. If the dual program is strictly feasible, i.e., there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi$. Then we have zero duality gap for the primal-dual pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual}.
%\end{theorem}
%\begin{proof}
%There exists an interior point $\psi^{*}   \in P^{\prime}$.  Here is the basic idea of the proof:  by Theorem \ref{thm:regular-duality}, the dual problem (\ref{eq:conlp-dual}) has finite limit value  $\hat{d}$ and $\hat{d} = z^{*}.$ Thus there is a sequence of $\psi_{k} \in P^{\prime},$ such that $\lim \sup_{k \rightarrow \infty} \langle d, \psi_{k} \rangle = z^{*}$ and $\lim_{k \rightarrow \infty} A^{*}(\psi_{k}) = \phi.$  Use the interior point $\psi^{*}$ to modify the sequence of $\psi_{k}$ to a new sequence $\eta_{k}$ where the $\eta_{k}$ satisfy $ A^{*}(\eta_{k}) = \phi,$  the $\eta_{k} \in  P^{\prime}$ for sufficiently large $k,$  and 
%$$
%\lim \sup_{k \rightarrow \infty} \langle  d, \eta_{k} \rangle > z^{*} - \epsilon
%$$
%for any $\epsilon > 0.$
% Next,  use the map  $T : P' \to \R^{(P')}_+$ from Theorem~\ref{theorem:new_express_dual} to construct a sequence of feasible solutions  $u(\eta_{k})$ to \eqref{eq:FDSILP} so that $\lim \sup_{k \rightarrow \infty} b(\eta_{k}) u(\eta_{k})  > z^{*} - \epsilon.$
% 
% \vskip 7pt
% 
% Okay, so how do we modify the $\psi_{k}$ into the $\eta_{k}$ using the interior point $\psi^{*}?$ Do the following ``trick'' from \cite{gartner-matousek}.
% 
% \begin{eqnarray*}
% \eta_{k} :=  (1 - \xi)\left(\psi_{k} + (A^{*})^{-1} ( \phi - A^{*}(\psi_{k} ) ) \right) +\xi \psi^{*}.
% \end{eqnarray*}
%\end{proof}





%\subsection{Slater Condition}

%\begin{example}
%Consider the following semidefinite program
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \quad  x
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right]
%+
%t
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right]
%&\succeq& 
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right]
%\end{eqnarray*}
%
%
%The dual problem is
%\begin{eqnarray*}
%\sup 
%\left<
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right] ,
%\psi   \right> \\
%{\rm s.t.} \qquad 
%\left<
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right] ,
%\psi   \right>  = 0\\
%\left<
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right] ,
%\psi   \right>  = 1 \\
%\psi \succeq 0
%\end{eqnarray*}
%Now formulate the \eqref{eq:SILP}.
%
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \qquad x 
%\left<
%\left[
%\begin{array}{cc}
%1 & 0 \\
%0 & 0
%\end{array}
%\right] ,
%\psi   \right> 
%+
%t
%\left<
%\left[
%\begin{array}{cc}
%0 & 0 \\
%0 & 1
%\end{array}
%\right] ,
%\psi   \right>
%&\ge&
%\left<
%\left[
%\begin{array}{cc}
%0 & -1 \\
%-1 & 0
%\end{array}
%\right] ,
%\psi   \right> 
%\end{eqnarray*}
%This simplifies to
%\begin{eqnarray*}
%\inf t && \\
%{\rm s.t.} \qquad  
%x \psi_{11} + t \psi_{22} 
%&\ge& -2 \psi_{12}
%\end{eqnarray*}
%This simplifies to
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad   z - t &\ge& 0 \\
%x \psi_{11} + t \psi_{22} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} > 0 \\
%x \psi_{11} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%t \psi_{22} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} = 0, \psi_{22} > 0 
%\end{eqnarray*}
%Project out the $t$ variable. This gives
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0  \\
%x \psi_{11} 
%&\ge&  -2 \psi_{12}, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%z  
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} =  0, \psi_{22} > 0 
%\end{eqnarray*}
%Now for the $\psi$ to be positive semidefinite, if either $\psi_{11} = 0$ or $\psi_{22} = 0$, the $\psi_{12} = 0$ so the system becomes
%\begin{eqnarray*}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0  \\
%x \psi_{11} 
%&\ge& 0, \quad \psi_{11} > 0, \psi_{22} = 0 \\
%z  
%&\ge&  0,  \quad \psi_{11} =  0, \psi_{22} > 0 
%\end{eqnarray*}
%Dividing the second inequality by the strictly positive $\psi_{11}$ gives
%\begin{eqnarray}
%\inf z && \\
%{\rm s.t.} \qquad  
%z + x  \frac{\psi_{11}}{ \psi_{22} } 
%&\ge&  -2  \frac{\psi_{12}}{ \psi_{22} },  \quad \psi_{11} > 0, \psi_{22} > 0   \label{eq:cone-I4}\\
%x 
%&\ge& 0, \quad \psi_{11} > 0, \psi_{22} = 0  \label{eq:cone-I2}\\
%z  
%&\ge&  0,  \quad \psi_{11} =  0, \psi_{22} > 0 \label{eq:cone-I3}
%\end{eqnarray}
%In this system, equations (\ref{eq:cone-I4}) correspond to the set $I_{4}$ in (\ref{eq:J_system}),  equations (\ref{eq:cone-I2}) correspond to the set $I_{2}$ in (\ref{eq:J_system}), and equations (\ref{eq:cone-I3}) correspond to the set $I_{3}$ in (\ref{eq:J_system}).
%So now 
%\begin{eqnarray*}
%\omega(\delta) = \sup \{ - \frac{2 (\psi_{12} + \delta \psi_{11})}{\psi_{22}}  \, : \,  \psi_{11}, \psi_{22} \ge 0\}
%\end{eqnarray*}
%Now look at slide IMG\_0083.jpg.  We argue you can take $\psi_{11} = 1.$  Since the matrix $\psi$ must be positive semidefinite, $\psi_{11} \psi_{22} - \psi_{12} \psi_{21} \ge 0.$  Then taking  $\psi_{11} = 1$ gives  $\psi_{22} - \psi_{12} \psi_{21} \ge 0.$ But the $\psi$ matrix is positive symmetric so $\psi_{22} \ge \psi_{12}^{2}.$  Then
%\begin{eqnarray*}
%\frac{-2 \psi_{12} - \delta}{\psi_{22}} \le  \frac{-2 \psi_{12} - \delta}{\psi_{12}^{2}}
%\end{eqnarray*}
%Optimizing by Calculus  gives $\psi_{12} = \delta$ and we get $(\delta) \le \frac{1}{\delta}.$
%\end{example}

%\vskip 10pt

%Some ideas: We want to avoid using Theorem 4.6.5 to prove the Slater result.  So it would seem at the minimum we need some kind of result such as:  {\it If the dual program (\ref{eq:conlp-dual}) is strictly feasible, i.e., there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi,$  then $I_{3}$ is not empty and $\sup_{h \in I_3}  \ge \lim_{\delta \rightarrow \infty}\omega(\delta).$ } 
%
%\vskip 7pt
%
%How about something even easier. Can we show:   {\it If the dual program (\ref{eq:conlp-dual}) is strictly feasible, i.e., there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi,$  then \eqref{eq:FDSILP} is feasible, or put another way $I_3$ is not empty.}


\subsection{Zero duality gap via an interior point condition}

%Assume throughout this section $X$ and $Y$ are  finite-dimensional spaces, and $P$ is reflexive\old{, and  $X = \R^n$} (note that any closed cone is reflexive because $Y$ is finite-dimensional). As before, identify $X$ with $\R^n$. 
The main result of this section demonstrates how the Fourier-Motzkin elimination procedure can be used to establish a ``Slater-like" theorem for conic programs. The result is well known. Alternate proofs can be found in the conic programming literature (see for instance Chapter~4 of \cite{gartner-matousek}).

Let $B(x, \epsilon) \subseteq \R^n$ denote the open ball of radius $\epsilon$ with center $x \in \R^n$.  Identify the objective linear functional $\phi \in X^{\prime}$ with the vector $c\in \R^n$.

\begin{lemma}\label{lem:open-mapping} Assume  $A' : Y' \to X'$ is surjective and there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = c$. Then there exists $\epsilon > 0$ and such that for all $\bar c \in B(c, \epsilon),$ there exists a  $\bar \psi \in P'$ such that  $\bar{c}^\top x \geq \langle d, \bar \psi \rangle$ is a constraint in~\eqref{eq:con-silp}.
\end{lemma}

\begin{proof}
For each $\psi \in P'$, the constraint in~\eqref{eq:con-silp} corresponding to $\psi$ is   $\sum_{j=1}^n x_j    \langle A(e^{j}), \psi  \rangle  \geq \langle d, \psi \rangle$. The left hand side of the inequality is the same as $\sum_{j=1}^n x_j    \langle e^{j}, A'(\psi)  \rangle = \langle x, A'(\psi)\rangle$. Since $A'$ is a linear map between finite-dimensional spaces, it is continuous and by assumption, surjective. By the Open Mapping theorem, $A'$ maps open sets to open sets. Since $\psi^* \in \intr(P')$ there exists an open ball $B^* \subseteq P'$ containing $\psi^*$. Thus, $A'(B^*)$ is an open set containing $c$. Therefore, there exists an $\epsilon > 0$ such that $B(c, \epsilon) \subseteq A'(B^*)$. Thus, for every $\bar c \in B(c, \epsilon)$, there exists $\bar\psi \in B^*$ such that $A'(\bar \psi) =\bar c$. Since all $\psi \in B^*\subseteq P'$ give constraints $\langle x,  A'(\psi)\rangle \geq \langle d, \psi\rangle$ in~\eqref{eq:con-silp}, for every $\bar c \in B(c, \epsilon)$ there is the  constraint $\bar c ^\top x = \langle x, A'(\bar\psi)\rangle \geq \langle d, \bar\psi\rangle$ in~\eqref{eq:con-silp}.
\end{proof}



\begin{theorem}[Zero duality gap via an interior point]\label{thm:slater}
If  the primal conic program~\eqref{eq:conlp-primal} is feasible and  there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = \phi$, then there  is a  zero duality gap for the primal dual pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual}. Moreover, the primal is solvable.
\end{theorem}

\begin{proof}
By hypothesis,  there exists $\psi^* \in \intr(P')$ with $A'(\psi^*) = c$ so the dual conic program~\eqref{eq:conlp-dual} is feasible.  Since~\eqref{eq:conlp-primal} is also feasible by hypothesis, feasibility  of~\eqref{eq:conlp-dual} implies  \eqref{eq:conlp-primal}  is both feasible and  bounded. Then by Remark~\ref{rem:surjective-assum}, it is valid to assume $A'$ is surjective. 
%\old{Since $c \neq 0$, we can assume (after a relabeling of variables) that $x_1$ has nonzero objective coefficient.}

\begin{claim} The variables $x_1, \ldots, x_n$ remain clean when  Fourier-Motzkin elimination is applied  to~\eqref{eq:con-silp}.
\end{claim}
\begin{proof}[Proof of Claim]\renewcommand{\qedsymbol}{} 
Since $A'(\psi^*) = c$, there is a constraint $c^\top x \geq \langle d, \psi^* \rangle$ in the system~\eqref{eq:con-silp}.   The constraint $-c^\top x + z \geq 0$ is also present when Fourier-Motzkin elimination is performed on a semi-infinite linear program. 
%\old{Thus, $x_1$ starts out clean by our assumption that $x_1$ has nonzero objective coefficient.} 
By Lemma~\ref{lem:open-mapping}, there exists $\epsilon > 0$ such that every $\bar c \in B(c, \epsilon)$ gives a constraint $\bar c^\top x \geq b'$ in~\eqref{eq:con-silp} where $b' = \langle d,\bar \psi\rangle$ with $A'(\bar\psi) = \bar c$. Thus, for any $\delta < \epsilon$, both $(c + \delta e^j)^\top x \geq  b^j_+$ and $(c - \delta e^j)^\top x \geq  b^j_-$ are constraints for every $j = 1, \ldots, n$, (where $b^j_+$ and $b^j_-$ are $\langle d,\psi^j_+\rangle$ and $\langle d,\psi^j_-\rangle$ respectively with $A'(\psi^j_+) = c + \delta e^j$ and $A'(\psi^j_-) = c - \delta e^j)$). \medskip

\noindent\underline{\em Case 1: $c_j = 0$ for all $j=1, \ldots, n.$}  In this case the constraints are  $\frac{\epsilon}{2}x_j \geq  b^j_+$ and $-\frac{\epsilon}{2}x_j \geq  b^j_-$ in the system. During Fourier-Motzkin, for each $j=1, \ldots, n$, the constraints $\frac{\epsilon}{2}x_j \geq  b^j_+$ and $-\frac{\epsilon}{2}x_j \geq  b^j_-$ remain in the system until variable $x_j$ is reached. This makes all variables $x_1, \ldots, x_n$ clean throughout the Fourier-Motzkin procedure.

\medskip

\noindent\underline{\em Case 2: $c_j \neq 0$ for some $j \in \{1, \ldots, n\}.$}  Relabel the variables such that $j = 1$ and  $c_1 \neq 0$. Note that coefficient of $x_1$ in $-c^\top x + z \geq 0$,  has opposite sign to the coefficient of $x_1$ in each pair of  constraints $(c + \frac{\epsilon}{2} e^k)^\top x \geq b^kj_+$ and $(c - \frac{\epsilon}{2} e^k)^\top x \geq b^k_-$ for $j =2, \ldots, n$. Clearly $x_1$ is clean, and when  $x_1$ is eliminated the constraint $-c^\top x + z \geq 0$  is aggregated with the constraints $(c + \frac{\epsilon}{2} e^k)^\top x \geq b^k_+$ and $(c - \frac{\epsilon}{2} e^k)^\top x \geq b^k_-$, for each $k = 2, \ldots, n$. This leaves the constraints $\frac{\epsilon}{2} x_k + z \geq  b^k_+$ and $-\frac{\epsilon}{2} x_j + z\geq  b^k_-$ in the system for $k =2, \ldots, n$, after $x_1$ is eliminated.  As in Case 1, these constraints remain in the system variable until $x_k$ is reached. This makes all variables $x_1, \ldots, x_n$ clean throughout the Fourier-Motzkin procedure.\quad $\dagger$
\end{proof}

Since variables $x_1, \dots, x_n$ are clean throughout the Fourier-Motzkin procedure, and~\eqref{eq:con-silp} is feasible (since \eqref{eq:conlp-primal} is feasible), the problem is feasible and tidy and  by Theorem~\ref{theorem:all-clean-system}, there is a zero duality gap between the pair~\eqref{eq:con-silp}-\eqref{eq:con-silp-lagrangian-dual-finite}, and~\eqref{eq:con-silp} is solvable. 
%By Theorems~\ref{theorem:new_express} and~\ref{theorem:new_express_dual}, 
This implies that there is zero duality gap for the pair~\eqref{eq:conlp-primal}-\eqref{eq:conlp-dual}, and the primal \eqref{eq:conlp-primal} is solvable.\end{proof}

%\old{Since all variables are clean throughout the Fourier-Motzkin procedure, $I_4$ is empty. This also implies $I_3 \neq \emptyset$ since $z$ can never be projected out. Thus $\omega(\delta) = -\infty$ for all $\delta$ and therefore $\sup_{h \in I_3}\{\tilde{b}(h)\} > \lim_{\delta\to \infty}\omega(\delta)$. Since the primal is feasible and bounded, the conditions of Theorem~\ref{theorem:zero-duality-gap} are satisfied, implying zero duality gap. Moreover, the hypothesis of Theorem~\ref{theorem:primal-solvability} is satisfied implying that the primal is solvable.}

\begin{remark}
Since the dual conic program~\eqref{eq:conlp-dual} is also a conic program, one can consider~\eqref{eq:conlp-dual} as a primal conic program.  In this case  the dual is~\eqref{eq:conlp-primal}.  By Theorem~\ref{thm:slater}, there is a zero duality gap between this primal-dual pair if there is  a point $x^*$ such that $A(x^*) - d \in \intr(P)$. Moreover, the dual is solvable. \quad $\triangleleft$
\end{remark}





==> karney-duffin.tex <==
% !TEX root = ../fm-paper-resubmit-again.tex
%\subsection{Application:  Further results for  semi-infinite linear programs}\label{s:app-countable}
%\subsection{Finite approximations to semi-infinite linear programs}\label{s:finite-approx}

%\begin{remark}
%Wolfe \cite{wolfe67} proposed a method for solving \eqref{eq:CP} using column generation.  See also Dantzig \cite{dantzig63}.  The restricted master of  Dantzig and  Wolfe corresponds to  a modified (CP-FDSILP) containing  a {\it finite} subset of columns.  At each step of the  Dantzig and Wolfe algorithm, a column with a negative reduced  is added to the current restricted master.    This results in  a new restricted master with one more column. 
%Dantzig \cite{dantzig63} proves that  the optimal value of the restricted master converges to the optimal value of the convex program \eqref{eq:CP} as the number of iterations (columns in the restricted master) goes to infinity.  By Theorem \ref{theorem:karney-countable}, it is valid to assume a countable number of constraints  in  (\ref{eq:convex-silp}). Dantzig's  result is  then immediate from   Corollary \ref{cor:karney-duffin-karlowitz}.    For every $n \in \N$, let $P_n$ denote the finite linear program derived from~\eqref{eq:convex-silp} using the constraints indexed by $\{1, \ldots, n\}$ and the same objective function. Let $v(P_n)$ denote its optimal value.  The dual of   $P_n$ is exactly the Dantzig and Wolfe restricted master with $n$ columns. By Corollary \ref{cor:karney-duffin-karlowitz}, $\lim_{n\to \infty} v(P_n) = v(\text{CP-FDSILP}).$  By Theorem~\ref{theorem:CP-FDSILP},  $v(\text{CP-FDSILP}) = v(\text{CP})$ and the result of Dantzig is immediate.  \hfill$\triangleleft$
%\end{remark}

\subsection{Additional sufficient conditions for zero duality gap}\label{s:app-countable}

By looking at the recession cone of~\eqref{eq:bounded-zero-duality-gap} it is possible gain further insights and discover useful sufficient conditions for zero duality gaps in general semi-infinite linear programs.   We show  results first discovered by Karney~\cite{karney81}  follow directly and easily from our methods.   The recession  cone of~\eqref{eq:bounded-zero-duality-gap} is  defined by the system
\begin{eqnarray}
-  c_{1} x_{1} -  c_{2} x_{2} - \cdots - c_{n} x_{n}    &\ge&   0  \label{eq:bounded-recession-cone-1}  \\
  a^{1}(i) x_{1} + a^{2}(i) x_{2} + \cdots + a^{n}(i) x_{n} \phantom{ + z} &\ge& 0 \quad  \text{ for } i \in I.   \label{eq:bounded-recession-cone-2}
\end{eqnarray}
%
Applying Fourier-Motzkin elimination to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} gives
\begin{eqnarray}
0 &\ge&  0 \quad \text{ for } h\in H_1\label{eq:defineH1-recession} \\
\tilde{a}^{\ell}(h) x_{\ell} + \tilde{a}^{\ell+1}(h) x_{\ell+1} + \cdots + \tilde{a}^{n}(h) x_{n} &\ge& 0 \quad \text{ for } h \in H_{2}.  \label{eq:defineH2-recession}
\end{eqnarray}
%
Following the notation conventions of Karney~\cite{karney81},  $K$ denotes the recession cone of \eqref{eq:SILP},  given by the inequalities~\eqref{eq:bounded-recession-cone-2} and  \old{The lineality space of $K$  is denoted by $M = K \cap (-K).$   } $N$ denotes  the null space of the objective function vector $c.$  
\old{
\begin{remark}\label{remark:nullspace_K_N}
 If  $K \cap N$ is a subspace,   then for any  $r \in K \cap N$,   $-r  \in (K \cap N)$.  Then both $r$ and $-r$ are in $K$.  This implies $r \in M.$ Therefore,  $K \cap N \subseteq M.$  This observation is used later in Theorem \ref{theorem:unbounded-recession-cone}. \hfill $\triangleleft$
 \end{remark} }
 

\begin{lemma}\label{lemma:strict-inequality}
If $H_2$ is nonempty in \eqref{eq:defineH2-recession}, then there exists a ray $r \in \R^n$ satisfying~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} with at least one of the inequalities in~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} satisfied strictly.
\end{lemma}
\begin{proof}
If  $H_2$ is nonempty, there is a  $k \ge \ell$ such that   $\tilde a^k(h)$ is nonzero for at least  one $h \in H_{2}$.   Since $x_{k}$ is a dirty variable,  the nonzero $\tilde a^k(h)$ are of the same sign for all $h \in H_{2}$. If the $\tilde a^k(h)$ are all nonnegative, then set $x_k = 1$ and $x_i = 0$ for $i \neq k$; if  the $\tilde a^\ell(h)$ are all nonpositive, then set $x_k = -1$ and $x_i = 0$ for $i \ne k$. This  solution to \eqref{eq:defineH1-recession}-\eqref{eq:defineH2-recession} satisfies at least one of the inequalities in \eqref{eq:defineH1-recession}-\eqref{eq:defineH2-recession} strictly. Since this is the projection of some $r$ satisfying~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, this $r$ must satisfy at least one inequality in~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} strictly, since all inequalities in \eqref{eq:defineH1-recession}-\eqref{eq:defineH2-recession} are conic combinations of inequalities in~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}.
\end{proof}
 \old{
 Next, for each $k = \ell, \ldots, n$, construct a nonzero solution of~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} as follows. For a given $\hat{k},$ set  $x_{\hat{k}} = \delta > 0$ and $x_{k} = 0$ for $k \neq \hat{k}$  if the nonzero elements $\tilde{a}^{\hat{k}}(h)$  are positive and  $x_{\hat{k}} = \delta < 0$ and $x_{k} = 0$ for $k \neq \hat{k}$  if the nonzero elements $\tilde{a}^{\hat{k}}(h)$  are positive.      Complete the solution for $x_{1}, \ldots, x_{\ell -1}$ as follows. When Fourier-Motzkin elimination is applied to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} in matrix order, at step $\ell - 1$, there is a system of inequalities
\begin{eqnarray*}
\hat{a}^{\ell - 1}(i) x_{\ell-1}+ \sum_{k=\ell}^{n} \hat{a}^{k}(i) x_{k} \ge 0, \quad i \in I(\ell - 1),
\end{eqnarray*}
 where $I(\ell - 1)$ is an index set for all the constraints in the system after projecting out variables $x_{1}$ through $x_{\ell - 2}.$ Fixing  the $x_{k},$ $k = \ell, \ldots, n$ as described above gives
 \begin{eqnarray*}
\hat{a}^{\ell - 1}(i) x_{\ell-1}+ \hat{a}^{\hat{k}}(i)  \delta  \ge 0, \quad i \in I(\ell - 1).
\end{eqnarray*}
At this step, both ${\cal H}_{+}(\ell - 1)$ and ${\cal H}_{-}(\ell - 1)$ are nonempty. Then the system of inequalities at this step with the fixed $x_{\ell}, \ldots, x_{n}$ is
 \begin{eqnarray*}
 x_{\ell-1} &\ge& -  \hat{a}^{\hat{k}}(i) \delta / \hat{a}^{\ell - 1}(i) , \quad i \in {\cal H}_{+}(\ell - 1)  \\
 x_{\ell-1} &\le&  \hat{a}^{\hat{k}}(i) \delta / \hat{a}^{\ell - 1}(i) , \quad i \in {\cal H}_{-}(\ell - 1)
\end{eqnarray*}
Then all feasible values of  $x_{\ell-1}$ are given by (assuming  without loss $\delta > 0$)
\begin{eqnarray*}
\delta  \sup \{ -\hat{a}^{\hat{k}}(i)  / \hat{a}^{\ell - 1}(i)  \, : \, i \in {\cal H}_{+}(\ell - 1) \}    \le  x_{\ell-1} \le  \delta  \inf \{ \hat{a}^{\hat{k}}(i)  / \hat{a}^{\ell - 1}(i)  \, : \, i \in {\cal H}_{-}(\ell - 1) \},
\end{eqnarray*}
and a feasible value is, without loss,  $x_{\ell - 1} = d_{\ell - 1} \delta$ where 
\begin{eqnarray*}
d_{\ell - 1} =  \inf \{ \hat{a}^{\hat{k}}(i)  / \hat{a}^{\ell - 1}(i)  \, : \, i \in {\cal H}_{-}(\ell - 1) \}.
\end{eqnarray*}
Recursing back in this fashion to variable $x_{1}$ gives a nonzero solution vector $r$
\begin{eqnarray}
r = \delta (d_{1}, \ldots, d_{\ell - 1}, 0, \ldots, 1, \dots, 0).  \label{eq:define-extreme-ray}
\end{eqnarray}
where the 1 is in component $\hat{k}.$
 The rays defined  in~\eqref{eq:define-extreme-ray}   for  $k = \ell, \ldots, n$ are obviously nonzero  and feasible to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}    for all $\delta > 0$.  Indeed,  by construction,  the rays $r,$ are extreme rays of~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, but this fact is not needed in the results that follow.}


%\vskip 10pt
%\texttt{Below is the original statement for the corollary, after that is the iff statement. The proofs of both are identical, because the original proof already had both directions of the argument.}
%\vskip 10pt
\old{\begin{corollary}\label{cor:bounded-recession-cone}
Assume that   $\gamma \in \R$ and there is a feasible solution value to \eqref{eq:SILP} that is less than or equal to $\gamma.$  If the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, then \eqref{eq:SILP} is tidy, the primal is solvable, and  there is a zero duality gap for the primal-dual pair \eqref{eq:SILP} and \eqref{eq:FDSILP}.
\end{corollary}

\begin{corollary}\label{cor:bounded-recession-cone}
\eqref{eq:SILP} is feasible and tidy if and only if there exists a $\gamma \in \R$ such that \eqref{eq:bounded-zero-duality-gap} is feasible and the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}
In particular, the ``if" direction implies \eqref{eq:SILP} is solvable and there is zero duality gap.
\end{corollary}

\begin{proof}
We prove this by showing that the feasible region defined by  system~\eqref{eq:bounded-zero-duality-gap} is bounded if and only if the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}.  The result then follows from Theorem~\ref{theorem:bounded-zero-duality-gap}.


($\Longrightarrow$)  We show  that if  the feasible region defined by~\eqref{eq:bounded-zero-duality-gap} is bounded, then~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}  has the zero vector as the unique solution.  Prove the contrapositive and assume $\overline{x}$ is a nonzero solution to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}.  By hypothesis,~\eqref{eq:bounded-zero-duality-gap} has a feasible solution $\hat{x}.$  Then $\hat{x} + \lambda \overline{x}$ is feasible to~\eqref{eq:bounded-zero-duality-gap} for all positive $\lambda$, so $\overline{x}$ nonzero implies   the feasible region defined by~\eqref{eq:bounded-zero-duality-gap} is unbounded.  

($\Longleftarrow$)  We show that if the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, then the feasible region defined by system~\eqref{eq:bounded-zero-duality-gap} is bounded.  Prove the contrapositive and assume the feasible region defined by~\eqref{eq:bounded-zero-duality-gap} is not bounded. Note that this implies there is a nonzero solution to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}. 
If~\eqref{eq:bounded-zero-duality-gap} is  not bounded, then  by Theorem \ref{theorem:region-boundedness},  Fourier-Motzkin elimination applied to~\eqref{eq:bounded-zero-duality-gap}   gives system~\eqref{eq:defineI1}-\eqref{eq:defineI2}  with   $H_{2}$  not empty. The values of the right hand side  have no effect on the elimination process. Therefore, Fourier-Motzkin elimination applied to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}  also results in a nonempty $H_{2}$ in  system~\eqref{eq:defineH2-recession}.   Then  the extreme rays defined in~\eqref{eq:define-extreme-ray} are nonzero solutions to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}. 
\end{proof}



\begin{theorem}\label{theorem:unbounded-recession-cone}
Assume  \eqref{eq:SILP} is feasible and that applying Fourier-Motzkin elimination to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}  gives~\eqref{eq:defineH1-recession}-\eqref{eq:defineH2-recession}.  If $r$ is a ray defined by~\eqref{eq:define-extreme-ray}, and $r$ is not an element of  the null space $N,$ then $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})$.
\end{theorem}

\begin{proof}
Assume $r$ is a ray defined in~\eqref{eq:define-extreme-ray} and $r$ is not in $N,$  the null space of $c.$ Then $\langle r,  c\rangle  \neq 0.$ By construction, $r$ is a ray of~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}  so $\langle r,  c\rangle  \neq 0$ and~\eqref{eq:bounded-recession-cone-1}  together imply  $\langle r,  c\rangle < 0.$  By hypothesis, \eqref{eq:SILP} has a feasible solution $\overline{x}.$ Then $\overline{x} + r$ is feasible for all $\delta > 0.$ This implies \eqref{eq:SILP} is unbounded so $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})=-\infty$ and there is a zero duality gap.
\end{proof}
}
\begin{theorem}\label{theorem:unbounded-recession-cone}
If \eqref{eq:SILP} is feasible and $K \cap N$ is a subspace, then  $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})$.
\end{theorem}


\begin{proof}
\underline{{\em Case 1: $H_{2}$ in~\eqref{eq:defineH2-recession} is empty.}} Observe that the columns in  systems~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} and~\eqref{eq:initial-system-obj-con}-\eqref{eq:initial-system-con} are identical for variables $x_{1}, \ldots, x_{n}$. This means if $x_k$ is eliminated when  Fourier-Motzkin elimination  is applied to one system, it  is eliminated in the other system. Since $H_{2}$ in~\eqref{eq:defineH2-recession} is empty,  \eqref{eq:SILP} is tidy. Then by Theorem~\ref{theorem:all-clean-system},  $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})$.

\underline{{\em Case 2:  $H_{2}$ in~\eqref{eq:defineH2-recession} is not empty.}} If $H_{2}$ is not empty, by Lemma~\ref{lemma:strict-inequality}, there exists a $r$ satisfying~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} such that at least one of the inequalities in~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} is satisfied strictly. If $c^T r < 0$  and  $r \in K$, then $v(\ref{eq:SILP}) = -\infty$.   Therefore \eqref{eq:FDSILP} is infeasible by weak duality and $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP}) = -\infty$. If  $c^T r = 0$ then the constraint~\eqref{eq:bounded-recession-cone-1} is tight at $r$ and so
%% this said strict before, but I don't agree 
$r\in N$. Then $r \in K \cap N$ which is a subspace by hypothesis.   Then  $-r \in K \cap N$.  This implies  $r \in K \cap -K$. But this means that $r$ satisfies all inequalities in~\eqref{eq:bounded-recession-cone-2} at equality and this contradicts the fact established for this case that at least one inequality in \eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} is strict.
\old{
 it either contains an index $h$ such that $\supp(\overline{u}^{h})$ contains the index for row~\eqref{eq:bounded-recession-cone-1} or it does not contain such an $h$.  Assume no such $h$ index exits.  Fourier Motzkin   elimination applied to (SILP) generates exactly the same set of multiplier vectors as Fourier-Motzkin elimination applied to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}.  Therefore, if $H_{2}$  in~\eqref{eq:defineH2-recession} does not contain an index for a multiplier vector with support containing the objective function row,  $J_{4}$ must be empty  when Fourier-Motzkin elimination is applied to (SILP).   This  implies $\lim_{\delta \rightarrow \infty} \omega(\delta) = - \infty.$ Since (SILP) is feasible, by Theorem \ref{theorem:zero-duality-gap} there is a zero duality gap.


Now    assume that there is an element $h \in H_{2}$ such that $\overline{u}^{h}$ has a positive multiplier for the row~\eqref{eq:bounded-recession-cone-1}.     In the row of~\eqref{eq:defineH2-recession}  indexed by $h,$ at least one $\tilde{a}^{k}(h)$   for  $k = \ell, \ldots, n$ is nonzero.  Assume without loss $\tilde{a}^{n}(h)$ is nonzero.  Consider the extreme ray   $\overline{r} = \delta(d_{1}, \ldots, d_{\ell - 1}, 0, \ldots, 1)$ of~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2} defined in~\eqref{eq:define-extreme-ray} .  There are two cases to consider.  The ray $\overline{r}$ is in the lineality space of $K$ or it is not. First assume $\overline{r}$ is in the lineality space of $K$.  For all $\delta > 0$ the solution $(d_{1} \delta, \ldots, d_{\ell - 1} \delta, 0, \ldots, \delta)$ has positive slack on aggregate constraint $h$. This means at least one constraint indexed by $\supp(\overline{u}^{h})$ must have positive slack. But if $\overline{r}$ is in the lineality space of $K$, the constraint with positive slack must be $-  c_{1} x_{1} -  c_{2} x_{2} - \cdots - c_{n} x_{n}   \ge   0$ and $\overline{r}$ is not in $N.$  Then by Theorem \ref{theorem:unbounded-recession-cone}, $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})$.

Now assume $\overline{r}$ is not in the lineality space of $K,$ that is $\overline{r} \notin M.$  There are two subcases. Either $\overline{r}$ is in $N$ or $\overline{r}$ is not in $N$.  If $\overline{r}$ is not in $N,$ then again by by Theorem \ref{theorem:unbounded-recession-cone}, $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP})$.  So assume $\overline{r}$ is in $N.$  Then  $\overline{r} \in K$ and $\overline{r} \in N$.  Therefore $\overline{r} \in K \cap N.$ By hypothesis $K \cap N$ is a subspace.  Then by  Remark  \ref{remark:nullspace_K_N},  $\overline{r} \in K \cap N \subseteq M.$  But $\overline{r}$ cannot be $M$  since we have assumed $\overline{r} \notin M.$  This is a contradiction, so this case cannot arise when $K \cap N$ is a subspace.  

Thus, when $K \cap N$ is a subspace, either $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP}) = -\infty$ and there is no duality gap, or  $H_{2}$ must be empty and there is no duality gap by Corollary \ref{cor:bounded-recession-cone}. }\end{proof}

\subsubsection{Finite approximation results}

Consider an instance of \eqref{eq:SILP} and the corresponding finite support dual~\eqref{eq:FDSILP}. %Apply Fourier-Motzkin elimination on the reformulation~\eqref{eq:initial-system-obj}-\eqref{eq:initial-system-con} to obtain~\eqref{eq:J_system}. 
%Let $v(\ref{eq:SILP})$ denote the optimal value of~\eqref{eq:SILP} and $v(\text{FDSILP})$ denote the optimal value of~\eqref{eq:FDSILP}. 
For any subset $J \subseteq I$, define $\text{SILP}(J)$ as the semi-infinite linear program with only the constraints indexed by $J$ and the same objective function, and $v(J)$  the optimal value of $\text{SILP}(J)$. For example, if $J$ is a finite subset of $I$, $\text{SILP}(J)$ is a finite linear program.

\begin{theorem}\label{theorem:finite-approx} If \eqref{eq:SILP} is feasible, then $v(\text{FDSILP}) = \sup\{v(J) : J \textrm{ is a finite subset of } I\}.$
\end{theorem}

\begin{proof}
We first show that $v(\text{FDSILP}) \leq \sup\{v(J) : J \textrm{ is a finite subset of } I\}$. \old{By hypothesis, \eqref{eq:FDSILP} is feasible. }By hypothesis,  \eqref{eq:SILP} is feasible and this  implies  by Corollary~\ref{cor:dual-optimal-value} that  $v(\text{FDSILP}) = \sup_{h \in I_3} \tilde{b}(h)$. 
Therefore, for every $\epsilon > 0$, there exists a $h^* \in I_3$ such that $v(\text{FDSILP}) - \epsilon \leq \tilde{b}(h^*)$. %Consider the Fourier-Motzkin multipler $u^{h^*}$ and let $J^* = \supp(u^{h^*})\setminus\{0\}$, where $\{0\}$ refers to the $0$-th constraint in~\eqref{eq:initial-system-obj}-\eqref{eq:initial-system-con}. 
By Lemma~\ref{lemma:feasible-FDSILP}\eqref{item:I3-property}, there exists a $v^{h^*}\in \R^{(I)}$ with support $J^*$ such that $\tilde{b}(h^*) = \langle b, v^{h^*} \rangle = \sum_{i \in J^*}b(i) v^{h^*}(i)$, and $\sum_{i \in J^*}a^k(i)v^{h^*}(i) = c_k$. Since~\eqref{eq:SILP} is feasible, $\text{SILP}(J^*)$ is feasible; let $\bar x$ be {\em any} feasible solution to this finite LP. Thus, 
$$
\begin{array}{rcl}
c^T\bar x & = &\sum_{k=1}^n c_k \bar{x}_k \\
&=& \sum_{k=1}^n(\sum_{i \in J^*}a^k(i)v^{h^*}(i))\bar{x}_k \\
&=& \sum_{i \in J^*}(\sum_{k=1}^n a^k(i)\bar{x}_k) v^{h^*}(i) \\
&\geq &\sum_{i\in J^*} b(i)v^{h^*}(i) \\
& = & \tilde{b}(h^*).
\end{array}
$$

Since this holds for any feasible solution to $\text{SILP}(J^*)$, $v(J^*) \geq \tilde{b}(h^*) \geq v(\text{FDSILP}) - \epsilon$. Thus, for every $\epsilon > 0$, there exists a finite $J^* \subseteq I$ such that $v(J^*) \geq v(\text{FDSILP}) - \epsilon$. Hence,  $v(\text{FDSILP}) \leq \sup\{v(J) : J \textrm{ is a finite subset of } I\}$.

Next we show that $v(\text{FDSILP}) \geq \sup\{v(J) : J \textrm{ is a finite subset of } I\}$. Consider any finite $J^*\subseteq I$. It suffices to show that $v(\text{FDSILP}) \geq v(J^*)$.     If $v(J^*) = -\infty$, then the result is immediate. So assume $v(J^*) > -\infty$. Then $\text{SILP}(J^*)$  is bounded.  Since  \eqref{eq:SILP} is feasible by hypothesis, $\text{SILP}(J^*)$  is also feasible. Then   by Theorem~\ref{theorem:finite-strong-duality}, there exists a $v^* \in \R^{J^*}$ such that $\sum_{i\in J^*}b(i)v^*(i) = v(J^*)$ and $\sum_{i\in J^*}a^k(i)v^*(i) = c_k$. Define $\bar v \in \R^{(I)}$ by $\bar v(i) = v^*(i)$ for $i \in J^*$ and $\bar v(i) = 0$ for $i \not\in J^*$. Thus, $\bar v$ is a feasible solution to~\eqref{eq:FDSILP} with objective value $v(J^*)$. Therefore, $v(\text{FDSILP}) \geq v(J^*)$.
\end{proof}

Theorem \ref{theorem:finite-approx} is used to prove a series of results by Karney~\cite{karney81}. Consider a semi-infinite linear program with countably many constraints, i.e., $I = \N$. For every $n \in \N$, let $P_n$ denote the finite linear program formed using the constraints indexed by $\{1, \ldots, n\}$ and the same objective function. Let $v(P_n)$ denote its optimal value.

\begin{corollary}\label{cor:karney-duffin-karlowitz}
If~\eqref{eq:SILP} is feasible with $I = \N$, then $\lim_{n\to \infty} v(P_n) = v(\text{FDSILP}).$
\end{corollary}

\begin{proof}
Since $\{1, \ldots, n\}$ is a finite subset of $I$, $v(P_n) \leq \sup\{v(J) : J \textrm{ is a finite subset of } I\} = v(\text{FDSILP}) <\infty$ where the equality follows from Theorem~\ref{theorem:finite-approx} and the ``$<$" follows from weak duality since \eqref{eq:SILP} is feasible. Since $v(P_n)$ is a nondecreasing sequence of real numbers bounded above, $\lim_{n\to \infty} v(P_n)$ exists and $\lim_{n\to\infty}v(P_n) \leq v(\text{FDSILP}).$
Next prove that $\lim_{n\to \infty} v(P_n) \geq v(\text{FDSILP})$. Observe that for any finite subset $J^* \subseteq I$ there exists an $n^* \in \N$ such that $J^* \subseteq \{1, \ldots, n^*\}$ and this  implies  $v(P_{n^*}) \geq v(J^*)$. Thus, $\lim_{n\to \infty} v(P_n) \geq \sup\{v(J) : J \textrm{ is a finite subset of } I\}$ = v(\text{FDSILP}) where the equality follows from Theorem~\ref{theorem:finite-approx}.
\end{proof} 

\begin{corollary}[Karney~\cite{karney81} Theorem 2.1]\label{cor:karney81} If the feasible region of~\eqref{eq:SILP} with $I = \N$ is nonempty and bounded, then $\lim_{n\to \infty} v(P_n) = v(\ref{eq:SILP}).$\end{corollary}
\begin{proof} This follows from Theorem~\ref{theorem:bounded-zero-duality-gap} and Corollary~\ref{cor:karney-duffin-karlowitz}.
\end{proof}

\begin{corollary}[Karney~\cite{karney81} Theorem 2.4]\label{cor:karney-theorem-2-4} If $\eqref{eq:SILP}$ with $I = \N$ is feasible and the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, then $\lim_{n\to \infty} v(P_n) = v(\ref{eq:SILP}).$
\end{corollary}

\begin{proof} 
If the zero vector  is the unique solution to the system~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}, then the recession cone of \eqref{eq:bounded-zero-duality-gap} is $\{0\}$ and  \eqref{eq:bounded-zero-duality-gap} is bounded for any value of $\gamma$ such that \eqref{eq:bounded-zero-duality-gap} is feasible (such a $\gamma$ exists because \eqref{eq:SILP} is feasible). The result then follows from Theorem~\ref{theorem:bounded-zero-duality-gap} and Corollary~\ref{cor:karney-duffin-karlowitz}.\end{proof}

\begin{corollary}[Karney~\cite{karney81} Theorem 2.5] \label{cor:karney-theorem-2-5} Assume \eqref{eq:SILP} with $I = \N$ is feasible and let $r$ be a ray satisfying~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}. If $r$ is not an element of  the null space $N,$  then $\lim_{n\to \infty} v(P_n) = v(\ref{eq:SILP}) = -\infty.$
\end{corollary}

\begin{proof} If  $r \in K$ and $r \notin N,$  then $c^T r <0$.   This implies $v(\ref{eq:SILP}) = -\infty$ and \eqref{eq:FDSILP} is infeasible by weak duality.   Then  $v(\ref{eq:SILP}) = v(\ref{eq:FDSILP}) = -\infty$ and the result  follows from Corollary~\ref{cor:karney-duffin-karlowitz}.\end{proof}

\old{
\begin{corollary}\label{cor:karney-theorem-2-5}[Karney~\cite{karney81} Theorem 2.5]  Assume \eqref{eq:SILP} is feasible and that applying Fourier-Motzkin elimination to~\eqref{eq:bounded-recession-cone-1}-\eqref{eq:bounded-recession-cone-2}  gives~\eqref{eq:defineH1-recession}-\eqref{eq:defineH2-recession}.  If $r$ is a ray defined by~\eqref{eq:define-extreme-ray}, and $r$ is not an element of  the null space $N,$  then $\lim_{n\to \infty} v(P_n) = v(\ref{eq:SILP}) = -\infty.$
\end{corollary}

\begin{proof}  This follows from Theorem~\ref{theorem:unbounded-recession-cone}  and Corollary~\ref{cor:karney-duffin-karlowitz}.\end{proof}
}

\begin{corollary}[Karney~\cite{karney81} Theorem 2.6]\label{cor:karney-theorem-2-6}  If \eqref{eq:SILP} is feasible and   $K \cap N$ is a linear subspace, then $\lim_{n\to \infty} v(P_n) = v(\ref{eq:SILP}).$
\end{corollary}

\begin{proof} 
This follows from Theorem~\ref{theorem:unbounded-recession-cone}  and Corollary~\ref{cor:karney-duffin-karlowitz}.\end{proof}


%\subsection{Moving from uncountable to countable}
%
%Corollaries \ref{cor:karney-duffin-karlowitz} and \ref{cor:karney-theorem-2-6} require that \eqref{eq:SILP} has a countable number of constraints, $I = \N$. Based on the work of Karney~\cite{karney81}, we show this assumption can be relaxed.    Let $J \subseteq I.$  Denote by (SILP(J)) the semi-infinite linear program obtained from \eqref{eq:SILP} by deleting from~\eqref{eq:SILP} all the constraints indexed $I \backslash J.$ Let $v(\text{SILP}(J))$ denote the corresponding optimal objective function value. Likewise for $\text{FDSILP}(J)$ and $v(\text{FDSILP}(J)).$  The objective of this section is show that when $I$ is uncountable, there exists a countable $J \subset I$ such that
%\begin{eqnarray*}
%v(\ref{eq:SILP}(J)) &=& v(\ref{eq:SILP}) \\
%v(\ref{eq:FDSILP}(J)) &=& v(\ref{eq:FDSILP})
%\end{eqnarray*}
%
%Our development duplicates Karney~\cite{karney85}.   The vector space $\R^{n + 1}$ under the usual topology is {\it separable} and therefore contains a countable sequence of vectors that is dense in $\R^{n + 1}.$   In fact, in $\R^{n + 1}$, any uncountable sequence $\{(\alpha^{i}, b(i))\}_{i \in I}$ contains a dense subsequence  $\{(\alpha^{i}, b(i))\}_{i \in J}$ with $J \subset I$ and $J$ countable.
%
%
%\begin{lemma}\label{lemma:karney-countable}
%If the  sequence of vectors $\{ (\alpha^{i}, b(i)) \}_{i \in J}$ in $\R^{n}$ is dense in $\{(\alpha^{i}, b(i)) \}_{i \in I}$ then
%\begin{eqnarray*}
%\{  x \, :  \,     \langle x, \alpha^{i}\rangle \ge b(i), \quad  i \in J \}  = \{  x \, :  \, \langle x, \alpha^{i} \rangle  \ge b(i),  \quad  i \in I\}. 
%\end{eqnarray*}
%\end{lemma}
%
%\begin{proof}
%Obviously, 
%\begin{eqnarray*}
%\{  x \, :  \, \langle  x,  \alpha^{i} \rangle  \ge b(i),  \quad  i \in I\} \subseteq \{  x \, :  \,     \langle x,  \alpha^{i} \rangle \ge b(i), \quad i \in J \} 
%\end{eqnarray*}
%
%\begin{eqnarray*}
%\{  x \, :  \,     \langle x,   \alpha^{i} \rangle \ge b(i), \quad i \in J \}  \subseteq \{  x \, :  \, \langle x,  \alpha^{i} \rangle  \ge b(i),  \quad  i \in I\}. 
%\end{eqnarray*}
%Prove the contrapositive. Assume there is an $\overline{x} \in \R^{n}$ and an $\hat{i} \in I$ such that $\langle \overline{x}, \alpha^{\hat{i}}\rangle  <   b(\hat{i})$.  Each $\alpha$ is an element of  $ (\R^{n})^{\prime},$  but   $\R^{n + 1}  \cong  (\R^{n})^{\prime}.$   Therefore, given  an $\overline{x} \in \R^{n},$  we can view  $\langle  \overline{x}, \alpha   \rangle - b$ as a continuous function of the variables $(\alpha, b)$  from  $\R^{n + 1}$   to $\R.$ Then there is a sufficiently epsilon ball around the point $(\alpha^{\hat{i}}, b(\hat{i}) )$ in the domain of this continuous function that contains an element of $h \in J$ such that $\langle \overline{x}, \alpha^{h} \rangle  <   b(h)$. This implies $\overline{x}$ is not in $\{  x \, :  \,     \langle x,   \alpha^{i} \rangle \ge b(i), \quad i \in J \} $.
%\end{proof}
%
%
%\begin{theorem}\label{theorem:karney-countable}
%Given a feasible and bounded semi-infinite linear program \eqref{eq:SILP},  there exists a countable set $J$, which is a subset of $I$, such that
%\begin{eqnarray*}
%v(\ref{eq:SILP}(J)) &=& v(\ref{eq:SILP}) \\
%v(\ref{eq:FDSILP}(J)) &=& v(\ref{eq:FDSILP})
%\end{eqnarray*}
%\end{theorem}
%
%
%\begin{proof}
%There exists an $J_{0} \subseteq I$ such that the sequence of vectors $\{ \alpha^{i}\}_{i \in J_{0}}$ is dense in the sequence $\{ \alpha^{i}\}_{i \in I}.$  By Lemma \ref{lemma:karney-countable} it follows that $v(\text{SILP}(J_{0})) = v(\ref{eq:SILP})$.
%
%Now construct $J$ from $J_{0}$ such that $v(\text{FDSILP}(J)) = v(\text{FDSILP})$.  Since \eqref{eq:FDSILP} is a maximization problem, for any $J \subseteq I,$  
%$v(\text{FDSILP}(J)) \le v(\text{FDSILP}).$    If $ v(\text{FDSILP}) = -\infty$ then $v(\text{FDSILP}(J)) \le v(\text{FDSILP})$  implies  $v(\text{FDSILP}(J)) = v(\text{FDSILP})$ and the result holds.  Assume $v(\text{FDSILP}) $ is finite.   It then sufficies to show $v(\text{FDSILP}(J)) \ge v(\text{FDSILP}).$   For each $n$ there is a feasible $u$ 
%
%Construct a sequence of sets $J_{n}$, $n = 1, \ldots, \infty$ as follows.  Given $n,$ there is a feasible solution $v^{n} \in \R^{(I)}$ such that $\sum_{i \in I} b (i) v^{n}(i) >   v(\text{FDSILP}) - \frac{1}{n}.$  Let $J_{n} \leftarrow J_{n-1} \cup \supp(v^{n}).$ Then $v(\text{FDSILP}(J_{n})) \ge  v(\text{FDSILP}) - \frac{1}{n}.$ Let $J = \cup_{k=0}^{\infty} J_{n}$.  Then $J$ is countable and  $v(\text{FDSILP}(J_{n})) \ge  v(\text{FDSILP})$ since  $v(\text{FDSILP}(J_{n})) \ge  v(\text{FDSILP}) - \frac{1}{n}$ for $n = 1, \ldots, \infty.$  Therefore  $v(\text{FDSILP}(J)) = v(\text{FDSILP}).$
%\end{proof}
%
%
%
%
%
%
%
%
%
%






==> sequence-space-projection.tex <==
% !TEX root = ../fm-paper-resubmit-again.tex

%\subsection{Sufficiency of Finite Support Duals}\label{s:sequence-space-projection}
%
%In Section \ref{s:silp-classification}, ``Dual Results,'' we used projection to prove results about zero duality gaps and strong duality for the semi-infinite linear program~\eqref{eq:SILP}. However, the dual problem \eqref{eq:FDSILP} was the finite support dual, not the full algebraic dual \eqref{eq:silp-lagrangian-dual}. Conceivably, there could be situations where there is a non-zero (even infinite) duality gap with respect to \eqref{eq:FDSILP}; whereas, one has zero duality gap with respect to (DSILP) or indeed other duals. We now show that when \eqref{eq:SILP} has countably many constraints, i.e., $I = \N,$ there is usually no loss of generality when considering the finite support dual. Another case where the finite support dual suffices is when $I$ is a compact Hausdorff space \cite{borwein1983adjoint}.
%
%More precisely, when we have countably many constraints in an instance of \eqref{eq:SILP}, we can consider the constraint space to be $\R^\N$, i.e., $b \in \R^\N$ and $a^k \in \R^\N$ for all $k=1, \ldots, n$. In this case, the algebraic Lagrangian dual \eqref{eq:silp-lagrangian-dual} and the finite support dual \eqref{eq:FDSILP} are the same. 
%%\old{The vector space $\R^\N$ is an ordered vector space using the partial order on $\R^\N$ given by $x \succeq  y$ if and only if $x(i) \geq y(i)$ for all $i \in \N$. }
%Define the cone
%\begin{eqnarray*}
%\R^{\N}_+ = \{  x \in \R^{\N} \, : \, x \geq 0\}.
%\end{eqnarray*}
%then the dual cone
%\begin{eqnarray*}
%(\R^{\N}_+)' = \{  \psi \in (\R^{\N})^{\prime} \, : \, \langle x, \psi \rangle \ge 0, \, \forall x \in  \R^{\N}_+ \}.
%\end{eqnarray*}
%
%The elements in $(\R^{\N}_+)'$ are known as the positive linear functionals on $\R^\N$.
%
%\begin{theorem}\label{thm:pos-functionals}
%For every $\psi \in (\R^{\N}_+)'$, there exists $u \in \R^{(\N)}$ such that $u(i) \ge 0$ for all $i \in \N$ and $\langle x, \psi \rangle = \sum_{i\in \N}x(i)u(i)$ for every $x \in \R^\N$. In other words, every positive linear functional on $\R^\N$ can be represented by a finite support dual element.
%\end{theorem}
%
%%\old{
%%Some observations:
%%
%%\begin{itemize}
%%\item $\R^{\N}$ is  a Riesz space  --  see bottom third of page 526
%%
%%\item the $\psi  \in \R^{\N}_+^{+}$ linear functionals are what HH call positive operators -- see page 325
%%
%%\end{itemize}
%%
%%\noindent {\bf Proof Technique:}
%%
%%\begin{itemize}
%%\item[1.]  Show $\R^{\N}$ is  a Fr\'{e}chet lattice -- just quote HH -- see the first paragraph on page 528 after Theorem 16.1. HH states:  ``We already know that $\R^{\N}$ equipped with the product topology is a completely metrizable locally convex-solid Riesz space.''  Then see page 349 which defines a Fr\'{e}chet lattice  as a completely metrizable locally solid Riez space.
%%
%%\item[2.]  Use Theorem 9.6 on page 350 of HH that states that states that every positive real linear functional on  a Fr\'{e}chet lattice is continuous
%%
%%\item[3.]  Combine 1. and 2. and argue that $\psi \in \R^{\N}_+^{+} $ is a continuous linear functional -- be precise here and specify the product topology
%%
%%\item[4.] Use Theorem 16.3 on page 528 of HH that states that the topological dual of the  Fr\'{e}chet lattice $\R^{\N}$ is the Riesz space of sequences of finite support.
%%
%%\item[3.]  By 3,  $\psi \in \R^{\N}_+^{+} $ is in the topological dual of $\R^{\N}$.  Conclude by 4. that $\psi$ is a sequence with finite support. 
%%\end{itemize}
%%
%%{\bf Red Flag:} when talking about  continuity be careful about  which topology we are talking about.  I  think we are talking about the product topology $\tau$ define on $\R^{N}$, but what is each $\tau_{i}$ for $i = 1, 2, \ldots$  I guess when you are talking about the product topology on $\R^{\N}$ each of the topologies $\tau_{i}$ defined on $\R^{1}$ are the usual topology of open intervals.  That at least seems to be the implied in the proof of Theorem 16.3 at the top of page 529.
%%
%%\vskip 7pt
%%}
%\begin{proof}
%Consider any $\psi \in (\R^\N)^\prime$, i.e.,  $\langle x, \psi \rangle \geq 0$ for all $x \geq 0$. We want to show that $\psi$ can be represented by a finite support linear functional.
%\begin{claim}\label{claim:finite_M}
%There exists $M \in \N$ such that for all $v \in \R^\N_+$ whose first $M$ components are zero, $\langle v, \psi \rangle = 0$.
%\end{claim}
%\begin{proof}
%Suppose no such $M$ exists. Then for every $n \in \N$ there exists $v_n \in \R^\N_+$ such that $\langle v_n, \psi \rangle > 0$ and the first $n$ components of $v_n$ are zero. Consider the sequence of vectors $\hat v_n = \frac{v_n}{\langle v_n , \psi \rangle}$ for $n \in \N$. Observe that $\langle \hat v_n, \psi\rangle = 1$ for all $n \in N$.
% Now, consider any vector $a \in \R^\N_+$ where $a(i) = \sum_{n \in \N} \hat v_n(i)$ = $\sum_{n = 1}^{i} \hat v_n(i) + \sum_{n > i} \hat v_n(i)$.  Since $\hat v_n(i) = 0$ for all $n > i$,    $\sum_{n > i} \hat v_n(i) = 0$. This implies  $\sum_{n \in \N} \hat v_n(i)$ is a finite sum and  therefore well-defined.   Given any $N \in \N$,   it follows  from the definition of $a(i)$,  that  $a(i) - \sum_{n=1}^{N} \hat v_n(i) = \sum_{n \in \N} \hat v_n(i) - \sum_{n=1}^{N} \hat v_n(i) = \sum_{n > N} \hat v_n(i)$.  However,  $\sum_{n > N} \hat v_n(i)  \geq 0$  since the $\hat v_n$ are in $\R^\N_+$.  This implies  $a - \sum_{n = 1}^N \hat v_n \geq 0$. 
% Thus, $\langle a - \sum_{n = 1}^N \hat v_n, \psi \rangle \geq 0$ for every $N \in \N$. By linearity of $\psi$, this implies that $\langle a, \psi \langle \geq \sum_{n=1}^N \langle \hat v_n, \psi \rangle = N$ for every $N \in \N$. But this means $\langle a, \psi \rangle$ cannot be a finite number, which is a contradiction.
%\end{proof}
%
%Let $M$ be the natural number from Claim~\ref{claim:finite_M}. Now let $e^i$ denote the element of $\R^\N$ with 1 in the $i$-th coordinate and $0$ everywhere else. Let $u \in \R^{(\N)}$ be a finite support element given as follows :
%$$
%u(i) = \left\{ \begin{array}{rl} \langle e^i, \psi \rangle & i \leq M \\ 0 & i > M\end{array}\right.
%$$
%
%We now claim that $\langle x, \psi \rangle = \sum_{i \in \N}u(i) x(i)$ for every $x \in \R^\N$. Observe that any $x \in \R^\N$ can be represented as $x = \sum_{i = 1}^M x(i)e^i + v$ where $v$ has zeros in its first $M$ components. Thus, by Claim~\ref{claim:finite_M}, $\langle v, \psi \rangle = 0$. Hence $\langle x, \psi\rangle = \sum_{i=1}^M x(i) \langle e^i, \psi \rangle + \langle v, \psi \rangle = \sum_{i \in \N}u(i) x(i)$.\end{proof}
%\begin{remark}\label{remark:anderson-nash-conjecture}
%This result resolves the conjecture of Anderson and Nash on page 66 and shows that we can never find an example with a positive duality gap in the space of finite support, but no duality gap in the space of the algebraic dual, when the constraint space is $\R^\N$. \hfill$\triangleleft$
%\end{remark}
%
%\subsection{Duality gaps in proper subspaces of $\R^\N$}
%
%Even though the finite support dual problem is the same as the algebraic Lagrangian dual problem when we view the primal constraint space as $\R^\N$, the situation is different if we consider problems with countably many constraints where the primal constraint space is  an ordered proper subspace of $\R^\N$. Consider two examples of such subspaces: $\ell_\infty$ which is the space of all bounded real sequences, and $c$ which denotes the space of all convergent sequences. Clearly, $c \subset \ell_\infty \subset \R^\N$. We extend the notion of positive linear functionals to these subspaces: a linear functional $\psi$ on any subspace $X \subseteq \R^\N$ is called a positive linear functional on $X$ if $\langle x, \psi \rangle \geq 0$ for all $x \in \R^{\N}_+ \cap X$. 
%%\old{The following lemma shows that the set of positive linear functionals on $c$ is strictly bigger than the set of finite support positive linear functionals. }
%\begin{lemma}\label{lem:limit-func}
%The functional $\langle x, \psi \rangle = \lim_{i\to \infty} x(i)$ is a positive linear functional on the space $c$. However, $\psi$ cannot be extended to positive linear functional on $\R^\N$, i.e., it cannot be extended to an element of $(\R^{\N}_+)' \subseteq (\R^\N)'$. In particular, $\psi$ cannot be represented by a sequence with finite support.
%\end{lemma} 
%
%\begin{proof}
%%
%If the positive linear functional $\psi$, could be represented by a sequence on  $\R^\N$ with finite support, then the nonzero elements in the sequence would have to be positive. Then $\psi$ would be an element of $ (\R^{\N}_+)^{\prime}$.  Therefore,  if   $\psi$  cannot be extended to an element of $(\R^{\N}_+)^{\prime}$, $\psi$ cannot  be represented by a sequence with finite support. We next show that such an extension is indeed not possible.
%
%
%Suppose to the contrary that $\phi$ is such an extension. We will now derive a contradiction. Let $\mathbf{1}$ be the all ones sequence. Then $\langle \mathbf{1}, \phi \rangle = \langle \mathbf{1}, \psi\rangle = 1$. Let $v = (n)_{n \in \N}$ be the sequence $(1,2,3, \ldots)$. Since $v$ is in the nonnegative orthant $\langle v, \phi \rangle = \alpha \geq 0$. Let $M = \lceil \alpha \rceil + 1$. Consider the sequence $m = (0,0,0, ..., M, M, M, \ldots)$ where the first $M-1$ entries are 0. Then $v - m$ is in the nonnegative orthant, but $\langle v-m, \phi \rangle = \langle v, \phi \rangle - \langle m, \phi \rangle = \alpha - \langle m, \psi \rangle = \alpha - M < 0$. \end{proof}
%
%Although positive linear functionals on the space $c$ cannot be extended to    $(\R^{\N}_+)'$, they can be extended to positive linear functionals on $\ell_\infty$, as shown in the lemma below. This lemma  uses a result about extending linear functionals on ordered vector spaces.  
%%%%  begin old
%\old{We first need to introduce some notions. A vector space $X$ is called an {\em ordered vector space} if it has a partial order $\succeq$ satisyfing 
%\begin{enumerate}
%\item $x \succeq y$ implies $x + z \succeq y + z$ for all $x, y, z \in X$.
%\item $x \succeq y$ implies $\alpha x \succeq \alpha y$ for all $\alpha \in \R_+$ and $x, y \in X$.
%\end{enumerate}
%An ordered vector space is called a {\em Riesz space} if it is also a lattice under the partial order. $\R^\N$, $\ell_\infty$ and $c$ are all Riesz spaces under the standard partial order $x \succeq y$ if and only if $x\geq y$. Suppose $X$ is a Riesz spce, and let $M$ be a subspace of $X$. We say that $M$ {\em majorizes} $X$ if for every $x \in X$, there exists $y \in M$ such that $y \geq x$.
%}
%
%%%%  end old
%
%We first need to recall the notion of a {\em core point}. Given a vector space $X$ and a subset $A \subseteq X$, a point $a \in A$ is called a core point of $A$ if for every $x \in X$, there exists $\epsilon > 0$ such that $a + \lambda x \in A$ for all $0 \leq \lambda \leq \epsilon$. Some authors call such a point an {\em absorbing point} or an {\em internal point}.
%
%\begin{lemma}\label{lem:limit-func-extend}
%Every positive linear functional on $c$ can be extended to a positive linear functional on $\ell_\infty$.
%\end{lemma}
%\begin{proof} 
% Let $C =  \R^{\N}_+  \cap \ell_\infty$ be the nonnegative cone in $\ell_\infty$.  Take the convergent sequence $\mathbf{1}$. This convergent sequence is an element of  $C \cap c$.  Also, $\mathbf{1}$ is a core point of $C$ in $\ell_\infty$.  To see that  $\mathbf{1}$ is a core point of $C$, take any $x = \{a_n\} \in \ell_\infty.$  
%Since $\{a_n\}$ is in  $\ell_\infty$,     $sup_n \{ |a_n| \} = M < \infty.$ Then $\mathbf{1}    +  \lambda \{ a_n \} \in C$ for all $\lambda \in (0, 1/M).$  Since $C$ has a core point,  apply the Krein-Rutman  (see, for example, Holmes~\cite{holmes}, page 20) variation on Hahn-Banach and conclude we can extend linear functionals defined on $ \R^{\N}_+  \cap c$ to $C$ on ordered vector spaces.\end{proof}
%
%\old{Observe that $c$ majorizes $\ell_\infty$ : for any $x \in \ell_\infty$, let $y\in c$ be the sequence whose every entry is $\lVert x \rVert_\infty$. By Theorem 8.32 in~Aliprantis and Border~\cite{hitchhiker} we can extend every positive linear functional on $c$ to a linear functional on $\ell_\infty$.}
%
%This phenomenon can create a duality gap if we restrict ourselves to the finite support dual elements, when working in the subspaces $\ell_\infty$ or $c$; whereas, when we use the full Lagrangian dual, we have no duality gap as discussed in the following paragraph.
%
%\begin{example}[Example~\ref{example:not-primal-optimal} revisited]
%In this example, recall that the optimal primal value is $0$. It is easy to see that the finite support dual for this semi-infinite linear program is infeasible: The objective coefficient of $x_1$ in the primal is $0$ and the coefficient of $x_1$ is strictly positive in the constraints, and so the only possible dual element satisfying the dual constraint correpsonding to $x_1$ is $u = 0$; however, the objective coefficient of $x_2$ is $1$ and thus, we cannot satisfy the dual constraint corresponding to $x_2$. This shows that using the finite support dual leads to an infinite duality gap. On the other hand, if we view the constraint space as $c$ (or $\ell_\infty$) instead of $\R^\N$, then the limit functional defined in Lemma~\ref{lem:limit-func} (respectively, its extension to $\ell_\infty$ by Lemma~\ref{lem:limit-func-extend}) gives an optimal dual solution with optimal value $0$, giving zero duality gap. \hfill$\triangleleft$
%\end{example}



